A classification of pseudo-Anosov homeomorphisms via geometric Markov partitions

We continue with the ideas of Bonatti-Langevin-Jeandenans towards a constructive and algorithmic classification of pseudo-Anosov homeomorphisms (possibly with spines), up to topological conjugacy. We begin by indicating how to assign to every pseudo-Anosov homeomorphism an abstract geometric type through a Markov partition whose rectangles have been endowed with a vertical direction; these are known as geometric Markov partitions. Such assignment is not unique, as it depends on the specific geometric Markov partition, and not every abstract geometric type is realized by a pseudo-Anosov homeomorphism. This poses interesting problems related to the algorithmic computability of the classification. The article contains three main results: $i)$ the geometric type is a total invariant of conjugacy, $(ii)$ a pictorial and combinatorial criterion for determining when a given geometric type is realizable by a pseudo-Anosov homeomorphism is provided, and $(iii)$ we describe an algorithmic procedure for determining when two geometric types correspond to topologically conjugate pseudo-Anosov homeomorphisms.

==> Intro/Subintro.tex <==
\section{Pseudo-Anosov homeomorphisms }

In this text, we define a surface as a topological manifold of dimension $2$. We assume these surfaces to be closed (compact and without boundary) and orientable unless otherwise stated. We use $\text{Hom}(S)$ to denote the set of homeomorphisms from $S$ to itself, and $\text{Hom}_+(S)$ to refer to the subset of automorphisms of $S$ that preserve orientation. The Nielsen-Thurston classification (\cite{thurston1988geometry}, \cite[Theorem 13.2]{farb2011primer}) establishes a trichotomy for each homeomorphism in $\text{Hom}_+(S)$: they are isotopic to one that is periodic, pseudo-Anosov, or reducible, with the latter being a combination of the first two. 
A pseudo-Anosov isotopy class contains a homeomorphism $f: S \to S$ that preserves a pair of transverse measured foliations $(\mathcal{F}^s, \mu^s)$ and $(\mathcal{F}^u, \mu^u)$ (\cite[Lemma 9.3]{fathi2021thurston}) in  such a manner, that $f$ dilates the transverse measure $\mu^s$ by a \emph{stretch factor} $\lambda > 1$ and contracts by $\lambda^{-1}$ the transverse measure $\mu^u$. Such foliations are the canonical models of its class in the space of measured foliations, and the respective homeomorphism $f$ is called pseudo-Anosov.  The singularities of $\cF^s$ and $\cF^u$ must necessarily be of saddle-type with $k > 3$ separatrices, and they are said to be $k$-prongs.  We will study a generalization of these homeomorphisms by allowing the foliations to have singularities with $1$-prong. These are called generalized pseudo-Anosov homeomorphisms in \cite[Exposition 13.1]{fathi2021thurston}. However, nowadays there are more general constructions of surface homeomorphisms that generalize one or another property of the canonical pseudo-Anosov models (\cite{Hall2004unimodal}, \cite{Andre2005extensions}, \cite{boyland2023unimodal}). Therefore, we prefer to simply call them pseudo-Anosov and reserve the term "generalized" for these more modern constructions. We usually say that $f$ is \textbf{p-A} homeomorphism. 


We must to study the set of \textbf{p-A} homeomorphism in a surface $S$ up topological conjugacy by orientation preserving homeomorphism and provide a classification of their conjugacy classes. 

\begin{prob}\label{Prob: Clasification}
	
The \emph{classification problem} for generalized pseudo-Anosov homeomorphisms can be divided into three fundamental components.

	\begin{enumerate}
		\item 	\textbf{Finite presentation:} This aspect aims to provide a concise and combinatorial description of the conjugacy classes that contain a generalized pseudo-Anosov homeomorphism. It can be further divided into the following sub-problems:
		\begin{itemize}
			\item[I)]\textbf{Combinatorial representation:} The objective of this problem is to establish a formal and precise association between every generalized pseudo-Anosov homeomorphism $f$ and a \emph{finite combinatorial object} denoted as $T:=T(f)$. This association is designed such that the same combinatorial object is linked to a pair of generalized pseudo-Anosov homeomorphisms if and only if they are topologically conjugated. It is important to note that the association may not be unique and $f$ can have multiple valid representations.
						
			\item[II)] \textbf{Combinatorial models:} Given a combinatorial information associated to a generalized pseudo-Anosov homeomorphism $f$, $T(f)$, we propose to reconstruct a pseudo-Anosov homeomorphism that is conjugate to $f$ using the information provided by $T(f)$. This problem represents a higher level of ambition compared to the previous point, since successfully achieving this reconstruction involves the combinatorial representation.

		
		\end{itemize} 
		
		\item \textbf{Realization:}The set of combinatorial objects forms a set denoted by $\mathcal{GT}$, and the subset of these objects associated with a pseudo-Anosov homeomorphism is referred to as the \emph{pseudo-Anosov class} and will be denoted by $\mathcal{GT}(p\AA)$. Generally, $\mathcal{GT}(p\AA)$ is a proper subset of $\mathcal{GT}$.
		
		The second problem is to provide a characterization and an algorithm for determining whether or not an abstract combinatorial information belongs to the pseudo-Anosov class. Ideally, we would like to set a time bound for the algorithm to provide an answer.
	
		\item \textbf{Algorithmic decidability:} A generalized pseudo-Anosov homeomorphism can have multiple combinatorial representations. The subsequent problem involves determining whether two combinatorial representations in the pseudo-Anosov class correspond to conjugate pseudo-Anosov homeomorphisms or not. Similar to the previous problem, our objective is to develop an algorithm that can efficiently determine, within finite and bounded time, whether two combinatorial representations represent the same conjugacy class.
		
	A more ambitious task is to identify a finite and distinguished family, denoted $\Theta[f]$, of the set of combinatorial objects associated with the pseudo-Anosov homeomorphism $f$. This family must satisfy three essential criteria: 
		\begin{itemize}
		\item $\Theta(f)$ must be computable from any other combinatorial object associated with $f$.
		\item $\Theta(f)$ must allow the computation of any other invariant $T(f)$ associated with $f$.
		\item $\Theta(f)$ must be, by contention,  the minimum set of combinatorial information that satisfies the previous items.
		\end{itemize}
	\end{enumerate}
\end{prob} 





Let $S$ be a closed and oriented surface, and let $f: S \rightarrow S$ be a generalized pseudo-Anosov homeomorphism. The combinatorial object associated with $f$ will be the \emph{geometric type} of a \emph{geometric Markov partition} of $f$. In the course of presenting our results, we will provide an explanation and overview of these concepts.
 
 \section{Presentation of results.}
 
 
 \subsection{Geometric Markov partitions and its geometric type.}
 

Let $S$ be a closed oriented surface, and let $f$ be a pseudo-Anosov homeomorphism with spines. We denote by $(\mathcal{F}^s,\mu^s)$ and $(\mathcal{F}^u,\mu^u)$ its invariant foliations equipped with their transverse measures. A \emph{rectangle} $R\subset S$ of $f$ is defined as a pair $(R,r)$, where $r$ is a (equivalence class of) continuous map $r: [-1,1]^2 \rightarrow S$ such that its image is $R$, i.e., $r([-1,1]^2)=R$. Moreover, $r$ is a homeomorphism on $(-1,1)^2$, and the pre-images of $\mathcal{F}^s$ and $\mathcal{F}^u$ under $r^{-1}$ correspond to the horizontal and vertical foliations, respectively, of the unit square. We identify two rectangles $r$ and $r'$ if there are mappings $\varphi_s,\varphi_u: [-1,1] \rightarrow [-1,1]$ such that $r'^{-1} \circ r = (\varphi_s,\varphi_u)$ and $\varphi_{s,u}$ are increasing homeomorphisms defined on the interval $[-1,1]$ (see Definition~\ref{Defi: rectangle}). The interior of $R$ is denoted as $\overset{o}{R}$ and corresponds to the restriction of $r$ to $(-1,1)^2$. Typically, when the parametrization is not necessary for the exposition, we refer to the image of $r$ simply as a rectangle.

A \emph{Markov partition}  $\cR=\{R_i\}_{i=1}^n$ of $f$ is a decomposition of the surface into a finite set of rectangles with disjoint interiors, satisfying the following property: if $\overset{o}{R_i}\cap f^{-1}(\overset{o}{R_j})\neq \emptyset$, then every connected component $C$ of $\overset{o}{R_i}\cap f^{-1}(\overset{o}{R_j})$ is the interior of a \emph{horizontal sub-rectangle} of $R_i$ (see Definition~\ref{Defi: vertical/horizontal sub rectangles}), and $f(C)$ is the interior of a vertical sub-rectangle of $R_j$.
  

The following result is a classical theorem for the case of pseudo-Anosov homeomorphisms without spines (see~\cite{fathi2021thurston}). In Chapter \ref{Section: Existence}, we provide a recipe for constructing Markov partitions for generalized pseudo-Anosov homeomorphisms¨. The advantage of our procedure is that it begins by selecting a point, and the rest of the construction follows an algorithmic approach.
  
\begin{coro*}[\ref{Coro: Existence adapted Markov partitions}]
Every generalized pseudo-Anosov homeomorphism admits Markov partitions.
\end{coro*}

 
\subsection{Finite presentations: The geometric type is a complete conjugacy invariant.}


If $R$ is a rectangle, the intersection $\mathcal{F}^s\cap R$ is referred to as the horizontal foliation of $R$, while $\mathcal{F}^u\cap R$ is its vertical foliation. The definition of a rectangle naturally provides an orientation for these foliations. By choosing an orientation for the vertical (unstable) foliation and assigning the unique orientation to the horizontal (stable) foliation, such that the parametrization $r$ restricted to the interior of the unit square, $r:(0,1)\times (0,1)\to \overset{o}{R}\subset S$, is an orientation-preserving homeomorphism. 
A \emph{geometric Markov partition} of $f$ is a Markov partition of the homeomorphism where a vertical orientation has been chosen for all the rectangles within it. In the book \cite{bonatti1998diffeomorphismes}, the authors associate to each geometric Markov partition a combinatorial information called \emph{geometric type}. Let us take a moment to review this concept. Throughout the rest of our presentation, we assume that all rectangles have been assigned orientations in their respective horizontal foliations, i.e, they are indeed, geometric Markov partitions. 



Let $f$ be a generalized pseudo-Anosov homeomorphism and let $\cR=\{R_i\}_{i=1}^n$ be a geometric Markov partition of $f$. The set of horizontal sub-rectangles of $R_i$, which are the connected components of the intersection $\overset{o}{R_i}\cap f^{-1}(\overset{o}{R_k})$ for some $k\in \{1,\cdots,n\}$, is labeled from \emph{bottom to top} according to the vertical orientation in $R_i$. We denote these sub-rectangles as $\{H^i_j\}_{j=1}^{h_i}$, where $h_i$ is the number of horizontal sub-rectangles of $R_i$. These particular rectangles are known as the \emph{horizontal sub-rectangles of the Markov partition} $\cR$. Similarly, the vertical sub-rectangles of $R_i$, whose interiors are the connected components of $\overset{o}{R_i}\cap f(\overset{o}{R_k})$ for some $k\in \{1,\cdots,n\}$, are labeled from \emph{left to right} according to the horizontal order of $R_i$ as: $\{V^i_l\}_{l=1}^{v_i}$, where $v_i$ is the number of vertical sub-rectangles of $R_i$. These specific rectangles are referred to as the  \emph{vertical sub-rectangles of the Markov partition} $\cR$.



The numbers $\{(h_i,v_i)\}_{i=1}^n$ determine two formal sets:

\begin{eqnarray}\label{Equa: Horizontal vertical sub}
\cH=\{(i,j): i\in\{1,\dots,n\}, j\in\{1,\dots,h_i\},\\
\cV=\{(k,l): k\in\{1,\dots,n\}, l\in\{1,\dots,v_k\}.
\end{eqnarray}
which represent the vertical and horizontal rectangles of the Markov partition, indexed according to the order within each rectangle. The homeomorphism $f$ induces a bijection, $\phi: \mathcal{H} \to \mathcal{V}$, between them. It is defined as $\phi(i,j) = (k,l)$ if and only if $f(H^i_j) = V^k_l$. Here, a first numerical obstruction arises in the set $\{(h_i,v_i)\}_{i=1}^n$:

\begin{equation}\label{Equa: same sum v-i h-i}
\sum_{i=1}^{n}h_i=\sum_{i=1}^{n}v_i.
\end{equation}

Each oriented vertical leaf of a sub-rectangle $H^i_j$ is sent by the function $f$ to a vertical leaf of $V^k_l$. We can compare the orientations of these leaves and define $\epsilon(i,j) = 1$ if the vertical orientations of $f(H^i_j)$ and $V^k_l$ coincide, and $\epsilon(i,j) = -1$ otherwise. This procedure determines the function:
\begin{equation}\label{Equation: same horizontal vertical}
\epsilon\colon \cH \rightarrow \{1,-1\}.
\end{equation}


The \emph{geometric type} of a geometric Markov partition $\cR$ packages all this information into a quadruple:

\begin{equation}\label{Equation: Geometric type}
T(\cR):=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi=(\phi,\epsilon)\colon \cH\to \cV\times\{-1,1\}).
\end{equation}



Later on, we will explain how to define an \emph{abstract geometric type} (Definition ~ \ref{Defi: abstract geometric type}). The set of abstract geometric types will be denoted by $\mathcal{GT}$. However, it is important to note that not every abstract geometric type corresponds to the geometric type of a geometric Markov partition of a pseudo-Anosov homeomorphism. The \emph{pseudo-Anosov class} of geometric types, denoted as $\mathcal{GT}(p\AA)\subset \mathcal{GT}$, consists of those geometric types $T$ for which there exists a generalized pseudo-Anosov homeomorphism with a geometric Markov partition $\mathcal{R}$ whose geometric type is $T$. This discrepancy is the reason for the realization problem in \ref{Prob: Clasification}.


In Chapter \ref{Chapter: TypeConjugacy}, the following theorem is proved, achieving a solution to \textbf{Item} $1.I)$ of the classification problem. It establishes that the geometric type serves as a complete invariant under topological conjugacy.

\begin{theo*}[\ref{Theo: conjugated iff  markov partition of same type}]
Let $f:S_f\rightarrow S_f$ and $g:S_g \rightarrow S_g$ be two generalized pseudo-Anosov homeomorphisms. Then, $f$ and $g$ have a geometric Markov partition of the same geometric type if and only if there exists an orientation preserving homeomorphism between the surfaces $h:S_f\rightarrow S_g$ that conjugates them, i.e., $g=h\circ f\circ h^{-1}$.
\end{theo*}



To prove Theorem~\ref{Theo: conjugated iff markov partition of same type}, we will construct a \emph{combinatorial model} of a pseudo-Anosov homeomorphism $f:S_f \to S_f$ with a Markov partition $\mathcal{R}$ of geometric type $T$. We will then demonstrate that $f$ is conjugated to this model. Essentially, the combinatorial model is obtained by taking the quotient of a sub-shift of finite type under an equivalence relation determined by the geometric type. Let us provide a brief overview of this construction.


 
 The geometric type $T$ determines the \emph{incidence matrix} $A:=A(T)$ of the Markov partition $\cR$. When the matrix $A$ has coefficients in $\{0,1\}$, it is called a \emph{binary matrix}, and we can define a symbolic dynamical system called, sub-shift of finite type $\sigma\colon \Sigma_A\to\Sigma_A$. Furthermore, it is possible to create a function $\pi_f:\Sigma_A \rightarrow S_f$ that depends on the homeomorphism $f$ and the Markov partition $\cR$ as follows: Let $(w_z)_{z\in \mathbb{Z}}=\underline{w}\in \Sigma_A$.
 
 
\begin{equation}\label{Equa: Projection}
\pi_f(\underline{w}):=\cap_{n\in \NN}(\overline{\cap_{z=-n}^n f^{-z}(\overset{o}{R_{w_z}})}).
\end{equation}
 
The map $\pi_f$ is the \emph{projection of the shift} with respect to the geometric Markov partition $(f, \mathcal{R})$. The projection associates each itinerary $\underline{w}=(w_z)_{z\in \mathbb{Z}}$ with a unique point $x$ on the surface $S$ such that $f^z(x)\in R_{w_z}$, i.e $x:= \pi_f(\underline{w}) $ follows the itinerary dictated by the code $\underline{w}$. The definition of $\pi_f$ is based on the following idea: the sets $\overset{o}{Q_n}=\cap_{z=-n}^n f^{-z}(\overset{o}{R_{w_z}})$ are open rectangles contained within the interior of $R_{w_0}$, and their diameters approach zero as $n$ tends to infinity. Consequently, the closure of $\overset{o}{Q_n}$ cannot simultaneously touch the two stable (or unstable) boundaries of $R_{w_0}$. As was said before, the intersection of the closures of all these rectangles, $\cap_{n\in \mathbb{N}} \overline{Q_n}$, corresponds to a unique point $\pi_f(\underline{w}):=x$ that follows the itinerary dictated by $\underline{w}$.


 It's important to mention that this is not the only way to define the projection. For instance, in \cite{fathi2021thurston}, the projection is given by $\pi_f(\underline{w}) = \cap_{z\in \ZZ} f^{-z}(R_{w_z})$. However, if we define $\pi_f$ in this manner, the projection may not always be a function as $\pi_f(\underline{w})$ is not necessarily a single point, except in cases where all the rectangles in $\cR$ are embedded.
 
The projection $\pi_f$ defined in Equation \ref{Equa: Projection} is a continuous, surjective, and finite-to-one map that acts as a semi-conjugation between the sub-shift of finite type $(\Sigma_A, \sigma)$ and the generalized pseudo-Anosov homeomorphism $f$. 
 


If two generalized pseudo-Anosov homeomorphisms $f: S_f \to S_f$ and $g: S_g \to S_g$ have Markov partitions $\cR_f$ and $\cR_g$ of the same geometric type $T$, they will share the same incidence matrix and thus have associated identical sub-shifts of finite type. This implies the existence of projections $\pi_f: \Sigma_A \to S_f$ and $\pi_g: \Sigma_A \to S_g$ that semi-conjugate the shift with the respective homeomorphisms. However, it is not clear how we can establish a direct conjugation between $f$ and $g$ based solely on these projections.



The main challenge in constructing a conjugacy between $f$ and $g$ lies in determining the correspondence between codes in $\Sigma_A$ that represent the same points on the surfaces $S_f$ and $S_g$. This correspondence is particularly challenging because the only known information that relates $f$ to $g$ is the geometric type of their respective partitions. Therefore, our analysis will be based solely on this combinatorial information.


We adopt the approach of introducing an equivalence relation $\sim_T$ in $\Sigma_A$, which is purely determined by the geometric type $T$. This relation defines equivalence classes that correspond to the codes in $\Sigma_A$ that project to the same point under $\pi_f$. The advantage of using the equivalence classes determined by $\sim_T$ is that they do not depend on the specific homeomorphism $f$ or a Markov partition $\cR$. This allows us to compare different generalized pseudo-Anosov homeomorphisms that share the same geometric type for their Markov partitions. In Chapter \ref{Chapter: TypeConjugacy}, we construct this equivalence relation, and Proposition \ref{Prop: The relation determines projections} establishes its key properties.

\begin{prop*}[\ref{Prop: The relation determines projections}]
	
	Let $T$ be a geometric type with an incidence matrix $A:=A(T)$ having coefficients in $\{0,1\}$, and let $(\Sigma_A,\sigma)$ be the associated sub-shift of finite type. Consider a generalized pseudo-Anosov homeomorphism $f:S\rightarrow S$ with a geometric Markov partition $\cR$ of geometric type $T$. Let $\pi_f:\Sigma_A \rightarrow S$ be the projection induced by the pair $(f,\cR)$. 
	


There exists an equivalence relation $\sim_T$ on $\Sigma_A$, algorithmically defined in terms of $T$, such that for any pair of codes $\underline{w},\underline{v}\in \Sigma_A$, they are $\sim_T$-related if and only if their projections coincide, $\pi_f(\underline{w}) = \pi_f(\underline{v})$.
\end{prop*}

Two codes $\underline{v}, \underline{v}\in \Sigma_A$ are $\sim_f$-related if $\pi_f(\underline{v}) = \pi_f(\underline{v})$ (recall that $f:S_f\to S_f$ is pseudo-Anosov). This relation determines the quotient space $\Sigma_f := \Sigma_A/\sim_f$ and is not difficult to see that $\Sigma_f$ is homeomorphic to $S_f$. A further consequence of Proposition \ref{Prop: The relation determines projections} is the following result, from which Theorem \ref{Theo: conjugated iff markov partition of same type} follows.
 

\begin{prop*}[\ref{Prop:  cociente T}]
Consider a geometric type $T$ in the pseudo-Anosov class, whose incidence matrix $A:=A(T)$ is binary. Let $f:S \rightarrow S$ be a generalized pseudo-Anosov homeomorphism with a geometric Markov partition $\cR$ of geometric type $T$.  Also, let $(\Sigma_A,\sigma)$ be the sub-shift of finite type associated with $A$ and denote by $\pi_f:\Sigma_A \rightarrow S$ the projection induced by the pair $(f,\cR)$. Then, the following holds:
	
	\begin{itemize}
\item The quotient space $\Sigma_T = \Sigma_A/\sim_T$ is equal to $\Sigma_f := \Sigma_A/\sim_f$. Thus, $\Sigma_T$ is a closed and orientable surface.
\item  The sub-shift of finite type $\sigma$ induces a homeomorphism $\sigma_T: \Sigma_T \rightarrow \Sigma_T$ through the equivalence relation $\sim_T$. This homeomorphism is a generalized pseudo-Anosov and topologically conjugate to $f: S \rightarrow S$ via the quotient homeomorphism $[\pi_f]: \Sigma_T = \Sigma_f \rightarrow S$
	\end{itemize}	
\end{prop*}



Let $g$ be any other generalized pseudo-Anosov homeomorphism with a geometric Markov partition of geometric type $T$. Then, $g$ is topologically conjugate to $\sigma_T$. Therefore, $f$ and $g$ are topologically conjugate.


\begin{defi*}[\ref{Defi: symbolic model}]
Let $T$ be a geometric type whose incidence matrix is binary. The dynamical system $(\Sigma_T,\sigma_T)$ is the \emph{combinatorial model of the geometric type} $T$.
\end{defi*}

The dynamical system $(\Sigma_T,\sigma_T)$ is constructed from the geometric type $T$, and it is topologically conjugate to $f$. Therefore, we have addressed \textbf{Item} $1.II$ of the Classification Problem \ref{Prob: Clasification} by demonstrating that the geometric type $T$ allows us to reconstruct a generalized pseudo-Anosov homeomorphism that is topologically conjugate to $f$. 

%%%%%%%%%%%



 
\subsection{The realization problem: The genus and the impasse}
 
An \emph{abstract geometric type} is defined as a quadruple $T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi:=(\phi,\epsilon))$, as described in Equation \ref{Equation: Geometric type}, where $n\in\NN{+}$, the numbers $h_i,v_i\in\NN_{+}$ satisfy the equality in Equation \ref{Equation: same horizontal vertical}, and $\phi$ is a bijection between the following sets.
 $$
 \cH(T):=\{(i,j)\in \NN: 1\leq i \leq n \text{ and } 1 \leq j \leq h_i\}
 $$
 and
 $$
 \cV(T):=\{(k,l)\in \NN: 1\leq k \leq n \text{ and } 1 \leq l \leq v_i\},
 $$
  additionally, $\epsilon:\cH(T) \rightarrow \{1,-1\}$ is an arbitrary function. These objects together form the set of \emph{abstract geometric types} denoted by $\mathcal{G}\mathcal{T}$.

As mentioned previously, an abstract geometric type $T$ belongs to the \emph{pseudo-Anosov class} of geometric types if there exists a generalized pseudo-Anosov homeomorphism  with a geometric Markov partition of geometric type $T$. The pseudo-Anosov class is denoted by $\mathcal{G}\mathcal{T}(p\AA)$. It is evident that $\mathcal{G}\mathcal{T}(p\AA)\subset \mathcal{G}\mathcal{T}$, and \textbf{Item} $II$ of Problem \ref{Prob: Clasification} seeks an algorithmic condition to determine whether an abstract geometric type belongs to the pseudo-Anosov class. Our approach to this problem is to translate it into the context of \emph{basic pieces} of Smale's surface diffeomorphisms.

 

The theory of geometric types was first introduced in the 1998 book \cite{bonatti1998diffeomorphismes} by Christian Bonatti, Rémi Langevin, and Emmanuelle Jeandenans. This work was followed by François Béguin's Ph.D. thesis \cite{beguin1999champs} and subsequent articles \cite{beguin2002classification} and \cite{beguin2004smale} published between 1999 and 2004. Together, these works provide a complete classification (in the sense of Problem 1) of the basic saddle-type pieces of Smale's diffeomorphisms on surfaces, as well as their invariant neighborhoods but excluding hyperbolic attractors and repellers. The definition of the geometric Markov partition and its geometric type for diffeomorphisms is very similar to the one given for pseudo-Anosov homeomorphisms, with the advantage that the Markov partition for the basic pieces consists of disjoint rectangles.  To apply the results obtained by these authors, our initial task is to establish a connection between Markov partitions for pseudo-Anosov homeomorphisms and those defined by saddle-type basic pieces on surfaces. Let's explore some key concepts in our discussion. 


Consider a geometric type $T$, and let $A$ be its incidence matrix with coefficients in ${0,1}$. We say that $A$ is \emph{mixing} if there exists a positive integer $n$ such that each coefficient $a_{ij}^{(n)}$ of the matrix $A^n$ is positive. When the incidence matrix $A$ is mixing, we can define a \emph{concretization} of $T$ \footnote{In fact, a weaker condition is needed, namely, that the geometric type does not have double $s,u$-boundaries. However, this property is deduced from the fact that $A(T)$ is mixing.}.

 A concretization of $T$ is represented by a pair $(\cR,\phi)$, where $\cR$ is a collection of disjoint rectangles $\{R_i\}_{i=1}^n$ (we can take $R_i:=[0,1]^2 \times \{i\}$), and $\phi$ is a piecewise-defined function. The function $\phi$ maps a collection of disjoint horizontal sub-rectangles $H_j^i\subset R_i$ (for each $(i,j)\in \cH(T)$) to a family of disjoint vertical sub-rectangles $V_l^k\subset R_k$ (for each $(k,l)\in \cV(T)$). Within each rectangle, $\phi$ is a homeomorphism that preserves the orientation and trivial foliations of the rectangles, furthermore, $\phi$ follows the combinatorial pattern specified by $T$. Specifically, if $\phi(i,j)=(k,l)$, then, $f(H_j^i)=V_l^k$,  and the orientation of the vertical foliations is preserved by $\phi$ if and only if $\epsilon(i,j)=1$.

A concretization provides a visual representation of the geometric type $T$, but it alone cannot determine whether $T$ corresponds to the geometric type of a geometric Markov partition of a saddle-type basic piece. However, if $T$ does correspond to the geometric Markov partition of a saddle-type basic piece of a diffeomorphism on a compact surface $S$ (with finite genus), it is crucial that such a surface contains the rectangles of a realization of $T$  and their images under the iterations of such diffeomorphism. 

To establish that $T$ is a geometric type corresponding to a geometric Markov  partition of a saddle-type basic pieces in $S$, it is necessary for a specific surface with boundaries and corners, known as an $m$-realizer of $T$ (described in Definition \ref{Defi: m realizer }), to be embedded in the surface $S$. We will now describe the main properties and definitions related to the $m$-realizer that are necessary to state our results.
 
 
Consider a concretization $(\{R_i\}_{i=1}^n,\phi)$ of $T$.  The union of these rectangles will be denoted as $\cR:=\bigcup_{i=1}^n R_i$.
The $m$-\emph{realizer} of $T$ is defined as the surface (with vertices and boundaries):
$$
\cR_m=\cup_{i=0}^m \cR\times \{i\}/(x,i)\sim(\phi^{-1}(x),i+1)
$$

together with the function $\phi_m(x,i)=(\phi(x),i+1)$ whenever it makes sense. 


The surface $\mathcal{R}_m$ has vertices and corners and supports $m-1$ iterations of the diffeomorphism $\phi_m$. These $m$-realizers determine a non-decreasing sequence $\{g_m\}_{m\in \mathbb{N}}$, where $g_m$ is the genus of the surface $\mathcal{R}_m$. The supremum of this sequence is defined as the \emph{genus of} $T$, denoted as $\text{gen}(T)$. The geometric type $T$ has \emph{finite genus} if $\text{gen}(T)<\infty$. Having finite genus is the first obstruction in realizing $T$ as the geometric type of a basic piece, and subsequently as the geometric type of a pseudo-Anosov homeomorphism.

The \emph{impasse property} of Proposition \ref{Prop: pseudo-Anosov iff basic piece non-impace} is quite technical (Definition \ref{Defi: Impasse geo}). For now, we won't explore it further to stay focused on the main exposition. The following Proposition is crucial for solving the realization problem. 

 \begin{prop*}[ \ref{Prop: pseudo-Anosov iff basic piece non-impace}]
	Let $T$ be an abstract geometric type. The following conditions are equivalent.
	\begin{itemize}
		\item[i)] The geometric type $T$ is realized as a mixing basic piece of a surface Smale diffeomorphism without impasse.
		\item[ii)] The geometric type $T$ is in the pseudo-Anosov class.
		\item[iii)] The geometric type $T$ satisfies the following properties:
		\begin{enumerate}
			\item  The incidence matrix $A(T)$ is mixing
			\item The genus of $T$ is finite
			\item $T$ does not have an impasse.
		\end{enumerate}
	\end{itemize}
\end{prop*}


To determine the realization of the geometric type in Problem \ref{Prob: Clasification}, it is necessary to demonstrate that each property listed in \textbf{Item} $iii)$ of Proposition \ref{Prop: pseudo-Anosov iff basic piece non-impace} can be determined algorithmically. This is achieved in the Preliminaries Chapter, specifically in Subsection \ref{Sec: Bonatti-Langevin theory}, where Proposition \ref{Prop: mixing+genus+impase is algorithm} establishes that the properties of mixing, finite genus, and impasse can be expressed in a purely combinatorial manner. This allows us to conclude the following theorem.

\begin{theo*}[\ref{Theo: caracterization is algoritmic}]
	There exists a finite algorithm that can determine whether a given geometric type $T$ belongs to the pseudo-Anosov class. Such algorithm requires calculating at most $6n$ iterations of the geometric type $T$, where $n$ is the first parameter of $T$.	
\end{theo*}


This resolves the problem of realization that we had set out to address.

\subsection{Algorithmic Decidability: The Béguin's Algorithm and Formal DA$(T)$}


To address \textbf{Item} $III$ of Problem \ref{Prob: Clasification} regarding algorithmic decidability, we utilize the \emph{Béguin's algorithm}. This algorithm, originally developed in \cite{beguin2004smale}, provides a solution for determining whether two geometric types represent conjugate basic pieces. Its essence can be summarized as follows:

\begin{theo*}[The Béguin's Algorithm]
Let $f$ be a Smale surface diffeomorphism and $K$ be a saddle-type basic piece with a geometric Markov partition $\mathcal{R}$ of geometric type $T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi_T)$. The steps of the algorithm are as follows:
\begin{enumerate}
\item Begin by defining the \emph{primitive geometric types of order} $n$ of $f$, denoted as $\cT(f,n)$, for all $n$ greater than a certain constant $n(f)\geq 0$.
\item Prove the existence of an upper bound $O(T)$ for $n(f)$ in terms of the number $n$ in $T$, i.e. $n(f)\leq O(T)$.
\item For every $n>n(f)$, there exist an algorithm to compute all the elements of $\cT(f,n)$ in terms of $T$.
\item Let $g$ be another Smale surface diffeomorphism and $K'$ be a saddle-type basic piece of $g$ with a geometric Markov partition of geometric type $T'$. Choose $n$ to be greater than or equal to the maximum of $O(T)$ and $O(T')$. After applying Step 3 of the algorithm, we obtain two finite lists of geometric types, $\cT(f,n)$ and $\cT(g,n)$. These lists will be equal if and only if $f$ is topologically conjugate to $g$ in some invariant neighborhoods of $K'$ and $K'$.
\end{enumerate}
\end{theo*}


As can be observed, the calculation of the upper bound $O(T)$ for $n(f)$ and the procedure in item 3 are the essential steps of the algorithm. We will revisit them at the end of this subsection. 

For now, let us explain how we address our problem by shifting the analysis to the formal \textbf{DA}$(T)$ (Definition \ref{Defi: Formal DA}). Consider a geometric type $T$ in the pseudo-Anosov class. According to Proposition \ref{Prop: pseudo-Anosov iff basic piece non-impace}, $T$ has finite genus. Interestingly, this condition is necessary and sufficient for $T$ to be realized as a basic piece of a Smale surface diffeomorphism. The \emph{formal derived from Anosov} of $T$ refers to this realization and is represented by the triplet:

\begin{equation}\label{Equa: DA of T}
 \textbf{DA}(T):=(\Delta(T),K(T),\Phi_T),
\end{equation}

The components are as follows: $\Delta(T)$ is a compact surface with boundary of finite genus, $\phi_T$ is a Smale diffeomorphism defined on $\Delta(T)$; and $K(T)$, the unique nontrivial saddle-type basic piece of $(\Delta(T),\Phi_T)$ with a Markov partition of geometric type $T$.  We call $\Delta(T)$ the \emph{domain} of the basic piece $K(T)$. It is a profound result of Bonatti-Langevin \cite[Propositions 3.2.2 and 3.2.5, Theorem 5.2.2]{bonatti1998diffeomorphismes} that the \emph{DA}$(T)$ is unique up to conjugacy and serves as a bridge between the realm of pseudo-Anosov homeomorphisms and the basic pieces of Smale surface diffeomorphisms.
 

Let $f$ a generalized pseudo-Anosov homeomorphism and $\cR$ a geometric Markov partition, a periodic point of $f$ that is in the stable (unstable) boundary of $\cR$ is a $s$-boundary point ($u$-boundary point). Let $f$ and $g$ be two generalized pseudo-Anosov homeomorphisms, and let $\cR_f$ and $\cR_g$ be geometric Markov partitions with geometric types $T_f$ and $T_g$, respectively.
 Let  $p(f)$ be the maximum period of  periodic points of $f$ on the boundary of $\cR_f$, and $p(g)$ be the maximum period of periodic points of $g$ on the boundary of $\cR_g$. Take $p = \max\{p(f), p(g)\}$.  We are going to construct  geometric Markov partitions $\cR_{\cR_f,\cR_g}$ of $f$ and $\cR_{\cR_g,\cR_f}$ of $g$ such that: 


\begin{itemize}
\item The set of periodic boundary points of $\cR_{\cR_f,\cR_g}$ ( $\cR_{\cR_g,\cR_g}$ ) coincides with the set of periodic points of $f$ ( $g$ ) whose period is less or equal than $p$.
\item Every periodic boundary point in $\cR_{\cR_f,\cR_g}$ is a \emph{corner point} i.e. is $u$ and $s$-boundary.
\end{itemize}

 These refined partitions are referred to as the \emph{compatible refinements} of $\cR_f$ and $\cR_g$, and their respective geometric types are denoted $T_{(\cR_f,\cR_g)}$ and $T_{(\cR_g,\cR_f)}$.
 
 
Two geometric types, $T_1$ and $T_2$, which can be realized as basic pieces, are considered to be \emph{strongly equivalent} if there exists a Smale diffeomorphism $f$ of a compact surface and a nontrivial saddle-type basic piece $K$ of $f$, such that $K$ has a geometric Markov partition of geometric type $T_1$ as well as a geometric Markov partition of geometric type $T_2$.  We have proven the following corollary , which establishes a connection between the formal \textbf{DA} of the geometric types of the compatible refinements and the underlying pseudo-Anosov homeomorphisms.
 
\begin{coro*}\ref{Coro: equivalence pA and DA}
	Let $f$ and $g$ be generalized pseudo-Anosov homeomorphisms with geometric Markov partitions $\cR_f$ and $\cR_g$ of geometric types $T_f$ and $T_g$, respectively. Let $\cR_{f,g}$ be the joint refinement of $\cR_f$ with respect to $\cR_g$, and let $\cR_{g,f}$ be the joint refinement of $\cR_g$ with respect to $\cR_f$, whose geometric types are $T_{f,g}$ and $T_{g,f}$, respectively.  Under these hypotheses: $f$ and $g$ are topologically conjugated through an orientation preserving homeomorphism if and only if $T_{f,g}$ and $T_{g,f}$ are strongly equivalent.
\end{coro*}

  
  In the proof we use the formal \textbf{DA} in the next manner: If $T_{(\cR_f,\cR_g)}$ and $T_{(\cR_g,\cR_f)}$ are strongly equivalent, then \textbf{DA}$(T_{(\cR_f,\cR_g)})$ and \textbf{DA}$(T_{(\cR_g,\cR_f)})$ are conjugate through a homeomorphism $h$. This homeomorphism induces a conjugation between $f$ and $g$.  Proposition \ref{Prop: preimage is Markov Tfg type} establish  that if $f$ and $g$ are topologically conjugate, then \textbf{DA}$(T_{(\cR_f,\cR_g)})$ has a Markov partition of geometric type $T_{(\cR_g,\cR_f)}$. Hence they  are strongly equivalent.
   

 Finally we use the Béguin's algorithm to determine if $T_{(\cR_f,\cR_g)}$ and $T_{(\cR_g,\cR_f)}$ are strongly equivalent. This provides a solution for the fist part of Item $III$ in Problem \ref{Prob: Clasification} through the following theorem.
  
  \begin{theo*}[\ref{Theo: algorithm conjugacy class}]
Let $T_f$ and $T_g$ be two geometric types within the pseudo-Anosov class. Assume that $f: S \rightarrow S_f$ and $g: S_g \rightarrow S_g$ are two generalized pseudo-Anosov homeomorphisms with geometric Markov partitions $\cR_f$ and $\cR_g$, having geometric types $T_f$ and $T_g$ respectively.  We can compute the geometric types $T_{f,g}$ and $T_{g,f}$ of their joint refinements through the algorithmic process described in Chapter \ref{Chap: Computations}, and the homeomorphisms $f$ and $g$ are topologically conjugated by an orientation-preserving homeomorphism if and only if the algorithm developed by Béguin determines that $T_{f,g}$ and $T_{g,f}$ are strongly equivalent.
  \end{theo*}
 
%%%%%%%%%%%%%%%%%%%%%%%


The second part of \textbf{Item} $1.III$ in Problem \ref{Prob: Clasification}, requires the identification of a finite and well-defined family of geometric types, denoted as $\Theta[f]$, for a given pseudo-Anosov homeomorphism $f$. This family should be computable based on any geometric type associated with $f$, enabling the computation of any other geometric type realized by $f$. Furthermore, it is desirable for this family to be as small as possible while fulfilling these requirements.
In this direction, we have obtained some partial results, which are outlined below.


Let $p$ and $q$ be two periodic points of $f$. Here, $F^s(p)$ represents a stable separatrice of $p$, and $F^u(q)$ represents an unstable separatrice of $q$. Proposition \ref{Prop: Recipe for Markov partitions} presents a topological algorithm that, given any point $z\in F^s(p)\cap F^u(q)$, generates a corresponding Markov partition $\cR_z$. The significance of this algorithm lies in the fact that, under certain conditions, the geometric type of $\cR_z$ remains constant along the orbit of $z$. To obtain a canonical family of geometric types for $f$, it becomes necessary to identify a distinguished set of points contained in $F^s(p)\cap F^u(q)$.




We begin by considering $p$ and $q$ as singular points of $f$, which are the more distinguished points that we can take. A point $z\in F^s(p)\cap F^u(q)$ is called \emph{first intersection point} of $f$ if the stable segment $(p,z]^s\subset F^s(p)$ and the unstable segment $(q,z]^u\subset F^u(q)$ intersect at a single point, $(p,z]^s\cap (q,z]^u={z}$ (see Definition \ref{Defi: first intersection points}). There exist a finite number of orbits of first intersection points as proved in Proposition \ref{Prop: Finite number first intersection points}. Clearly, a conjugation between pseudo-Anosov homeomorphisms maps first intersection points to first intersection points (see Theorem \ref{Theo: Conjugates then primitive Markov partition}) and therefore are invariant under conjugation. This property allows us to define: a natural number that is constant for the entire conjugacy class of $f$, $n(f)\geq 0$ , such that for every integer $n\geq n(f)$ and every first intersection point $z$, there exists a Markov partition $\cR(n,z)$ of $f$ associated to these two parameters.  The Markov partitions constructed in this manner are referred to as \emph{primitive Markov partition} of order $n$ of $f$. The collection of all these partitions is denoted by $\cM(f,n)$. They have the following property.


\begin{coro*}[\ref{Coro: Finite orbits of primitive Markov partitions}]		
	Let $f$ be a generalized pseudo-Anosov homeomorphism, and let $n\geq n(f)$. Then, there exists a finite but nonempty set of orbits of primitive Markov partitions of order $n$.
\end{coro*}


Our Theorem \ref{Theo: Conjugated partitions same types} states that a Markov partition and its iterations have the same geometric type. As a consequence, we have the following Theorem

\begin{theo*}[\ref{Theo: finite geometric types}]
	Let $f$ a generalized pseudo-Anosov homeomorphism. The set 
	$$
	\cT(f,n) = \{T(\cR): \cR \in \cM(f,n)\}
	$$ 
	is finite for every $n \geq n(f)$. These geometric types are referred to as \emph{primitive types} of order $n$ for $f$.
\end{theo*}


%%%%%%%%%%







Each of these families is a finite invariant under conjugation. If $f$ and $g$ are conjugate generalized pseudo-Anosov homeomorphisms, Corollary \ref{Coro: n(f) conjugacy invariant} establishes that $n(f)=n(g)$ and its set of \emph{canonical types} coincides too:
$$
\Theta[f]:=\cT(f,n(f))=\cT(g,n(g))=\Theta[g]
$$
Hence this  is a finite total invariant of the conjugation of $f$. They represent the finite presentation of \textbf{Item} $1.III$ in Problem \ref{Prob: Clasification}. Among the families of \emph{primitive types}, they are the minimum with  respect to the parameter $n$. 

At present, we are unable to compute the invariant $\Theta[f] := \cT(f,n(f))$ from any other geometric type or, in general, all geometric types associated with a conjugacy class as required by the \textbf{III} of Problem \ref{Prob: Clasification}. However, we can compute primitive geometric types of sufficiently large order. We believe it would be interesting to expand our theory and compute $\Theta([f])$, but this is still a work in progress.

We have concluded the presentation of the results in this thesis. Next, we will provide a brief survey of the results and perspectives surrounding the classification of pseudo-Anosov homeomorphisms. This is not an exhaustive bibliography, but rather an attempt to position our work within the context of the field.

==> Intro/clasifications.tex <==
\section*{Other classifications} 

The problem of classifying pseudo-Anosov homeomorphisms has been considered from different perspectives. In this section, we will discuss various results and approaches, in order to place our work within the current landscape of the mathematics. The conjugacy class and isotopy classes refer to the equivalence classes determined by topological conjugacy and isotopy, respectively.

\subsection{Lee Mosher: The classification of pseudo-Anosov}

In his 1983 thesis \cite{mosher1983pseudo} and the 1986 article \cite{mosher1986classification}, Lee Mosher classifies pseudo-Anosov homeomorphisms on a given closed and oriented surface $S$ equipped with a finite set of marked points $P$. To achieve this, Mosher considers the action of the mapping class group $\mathcal{M}(S,P)$ on a directed graph $\tilde{\mathcal{G}}(S,P)$, where each vertex represents a cellular decomposition of the surface with a single vertex and a distinguished sector around such vertex. The directed edges of $\tilde{\mathcal{G}}(S,P)$ correspond to elementary moves that transform one decomposition into another.


The mapping class group acts freely on the graph $\tilde{\mathcal{G}}(S,P)$, and the quotient yields a graph $\mathcal{G}(S,P)$ whose fundamental group is the mapping class group. Consequently, an element of the mapping class group can be represented by a cycle of directed edges in this graph. Each connected component of $\mathcal{G}(S,P)$ can be labeled using what Mosher refers to as \emph{polygonal types}, which essentially correspond to the list of polygons involved in the decomposition. It is worth noting that for a fixed genus of $S$ and a fixed number of marked points, there exists a finite number of polygonal types. Therefore, $\mathcal{G}(S,P)$ has a finite number of connected components.
 


Given a marked point-preserving pseudo-Anosov homeomorphism that fixes each of its  singularities and each of the separatrices of its singularities, Mosher define its \emph{singularity type}, which is determined by the number of interior singularities with $n$-prongs ($n \geq 3$) and marked singularities with $m$-prongs ($m \geq 1$). For each singularity type, he assigns a finite set of polygonal types of cellular decomposition to the pseudo-Anosov. His main result asserts that, for these polygonal types of cellular decomposition, the isotopy class of the pseudo-Anosov corresponds to a finite and explicit number of loops (cycles) on the graph $\mathcal{G}(S,P)$. Each of these loops has a finite combinatorial description, resulting in a finite number of canonical combinatorial descriptions for the pseudo-Anosov, they are called  \emph{pseudo-Anosov invariants.}


Thus, given two marked point-preserving pseudo-Anosov homeomorphisms that fix each of the separatrices of the singularities, they are conjugate if and only if their pseudo-Anosov invariants are the same. Mosher himself emphasizes that he does not know if his classification extends to a classification of all pseudo-Anosov homeomorphisms (without the assumption of fixing the separatrices).


As we have seen, Mosher's perspective and the one presented here are quite different. The distinction starts with the definition of a pseudo-Anosov homeomorphism. For Mosher, it is an isotopy class characterized by its action on a cell decomposition. In this thesis, we define a pseudo-Anosov homeomorphism through a Markov partition.  On which surface does it lay? What types of singularities does it possess? This information can be deduced from the geometric type of the partition, using a simple algorithm. Applying Mosher's result to a pseudo-Anosov homeomorphism defined by a geometric type of Markov partition seems to be a challenging task. However, a preliminary corollary, which we cite below, allows us to determine the singularity type of the pseudo-Anosov homeomorphism, which is a necessary piece of information for Mosher's result.

\begin{coro*}[\ref{Coro: Algorithm to Euler characteritic}]
	Let $T$ be a geometric type of the pseudo-Anosov class, and let $f:S\rightarrow S$ be a generalized pseudo-Anosov homeomorphism with a geometric Markov partition of type $T$. There exists a finite algorithm that, given $T$, determines the number of singularities of $f$ and the number of stable and unstable separatrices at each singularity and subsequently the genus of $S$.
\end{coro*}





 
 
 
 \subsection{The Bestvina-Handel Algorithm}
 
  

Let $S$ be a closed and oriented surface with marked points $P$. The objective of Bestvina and Handel in the article \cite{bestvina1995train} is to provide an algorithmic proof of the Handel-Thurston classification theorem for homeomorphisms in Hom$_+(S, P)$. In other words, given a homeomorphism $f$, their goal is to determine whether $f$ belongs to the isotopy class of a reducible, periodic, or pseudo-Anosov homeomorphism.


The article presents two main theorems which we will discuss below. These theorems are initially proven for surfaces with a single marked point and later extended to surfaces with a finite set of marked points. To facilitate the understanding of their results, we will provide an intuitive introduction to the key concepts involved.


A \emph{fibered surface} is a compact surface $F\subset S$ with  boundary that can be decomposed into arcs and polygons. These polygons are called \emph{junctions}, and the regions foliated by arcs are referred to as \emph{stripes}. We say that $F$ is \emph{carried} by a homeomorphism $f$ if $f$ maps $F$ into itself (up to isotopy) and sends the set of junctions to the set of junctions, as well as every stripe to the union of stripes.

If we collapse the fibered surface $F$, we obtain a graph $\cG$ where the vertices are the junctions and the edges are the stripes of $F$. If $F$ is carried by $f$, the homeomorphism induces a map on the graph $g:\cG\rightarrow \cG$ which sends vertices to vertices, and each 
edge to an edge-path. The map $g$ and the homeomorphism $f$ are irreducible if the incidence matrix of $g$ is irreducible and $\cG$ have no vertex of valence $1$ or $2$. Finally the growth rate of the map $g:\cG \to \cG$ is defined as the Perron-Frobenius eigenvalue of the incidence matrix of $g$, denoted by $\lambda(F,f)\geq 1$.

If every iteration of $g$ sends each edge of $\cG$ along a path without backtracking, and satisfy another technical condition of how the edge path cross every vertex, we say that $g$ is \emph{efficient} (see  \cite[Lemma 3.1.2]{bestvina1995train}). 
n

The first theorem of the authors establishes a dichotomy for $f$: it is either periodic or it carries an efficient fibered surface. This dichotomy forms the basis of their subsequent steps in the classification algorithm.
 
 \begin{theo*}[B-H, Theorem 3.1.3 ]
Every homeomorphism on a once punctured surface is isotopic, relative to the puncture, to one that is either reducible or carried by an efficient fibered surface.
 \end{theo*}


The proof follows an algorithmic approach. A spine of $S$ is a CW-complex $\cG$ contained in $S$ such that $S$ deformation retracts to $\cG$. The authors suggest starting with a regular neighborhood $F$ of a spine $G$ that naturally has a fibered surface structure. After that they perform an isotopy of $f$ to ensure that $F$ is carried by the homeomorphism. Then Bestvina and Handel follow the philosophy: the growth rate of the map $g$ is a measure of how close we are to an efficient fibered surface. The smaller the growth rate, the more efficient the carrier.

The algorithm described in \cite[Section 3]{bestvina1995train} is used to prove Theorem 3.1.3. It involves modifying the homeomorphism $f$ and the fibered surface $F$. Each step of the algorithm either reduces the growth rate of the induced map or maintains it at the same level as the previous step. The algorithm includes isotopies of $f$ and collapsing certain sub-graphs of $\mathcal{G}$, resulting in natural modifications of $F$.

It is proven that the algorithm terminates in finite time if $f$ is reducible, or it continues until an efficient carried surface is obtained. The algorithm terminates because the set of growth rates of non-negative integer matrices of bounded size is a discrete subset of $[1, \infty)$. As we decrease the growth rate of $g$, either $g$ becomes efficient, or we find a reduction and the algorithm stops. Next, Bestvina and Handel present the following result:

\begin{theo*}[B-H, Theorem 3.1.4 ]
If a homeomorphism $f:S\to S$ of a once-punctured surface is carried by an efficient fibered surface, then $f$ is isotopic, relative to the puncture, to a homeomorphism that is either periodic, reducible, or pseudo-Anosov.
\end{theo*}
 
   
 To prove Theorem 3.1.4, Bestvina and Handel utilize the concept of \emph{train tracks}. Like the  fibered surface is efficient, the map $g$ has a incidence matrix with growth rate greater than or equal to 1. In Section 3.3 of \cite{bestvina1995train}, the proof is divided into two cases
  
  \begin{itemize}
  	\item If $\lambda(F,f)=1$, it is observed that the homeomorphism is isotopic to a periodic one.
  	\item If $\lambda(F,f)>1$, either they can construct an $f$-invariant train track in finite time, or they find a reduction of $f$ (in which case $f$ is reducible).
  \end{itemize}

The second point is addressed in Section 3.4. There, they assume the existence of the $f$-invariant train track and use it to construct a Markov partition for the homeomorphism. Subsequently, they obtain the invariant foliations of $f$, establishing that $f$ is isotopic to pseudo-Anosov.

In their examples, the authors \cite[Section 6]{bestvina1995train} illustrate the initial step of the algorithm, which involves decomposing $f$ into Dehn twists. This serves as the input information for their algorithm.

An interesting question arises: given a geometric type $T$ in the pseudo-Anosov class, how can we find a decomposition of the underlying pseudo-Anosov homeomorphism into Dehn twists? Conversely, if we have a decomposition of $f$ into Dehn twists, can we calculate a geometric type associate of $f$? We think  is possible that the machinery of train-tracks, utilized to construct the Markov partition of $f$, could provide a solution to the last question.

 

Lastly, the authors do not explicitly discuss the problem of conjugacy. It is not clear to us how their algorithm can be used to determine if two pseudo-Anosov homeomorphisms are topologically equivalent, although it is possible that with further investigation, this could be achieved.


 \subsection{Jerome Los's Approach: The $n$-Punctured Disk and the Braid Group }
 
 The intimate relation between the mapping class group of the $n$-punctured disk and the Braid groups is exploited by Jerome Los in \cite{los1993pseudo} to provide a finite algorithm for determining whether an isotopy class (of the punctured disk) contains a pseudo-Anosov element.
 
 \begin{theo}[Los, J. \cite{los1993pseudo}]
Given a braid $\beta\in B_n$ defining an isotopy class $[f_{\beta}]$ of orientation-preserving homeomorphisms of the punctured disc $D_n$, there exists a finite algorithm which enables one to decide whether $[f_{\beta}]$ contains a pseudo-Anosov element. In the pseudo-Anosov case, the algorithm gives an invariant train track and the dilatation factor.
 \end{theo}

The train tracks are graphs that were introduced to simplify the description of the measured foliations on a surface. The author considers an even simpler graphs called \emph{skeleton graph}. The spirit of their algorithm is to consider all the possible maps induced on these graphs by some elements of the isotopy class $[f_{\beta}]$.

J. Los is able to simplify the problem by reducing it to a finite set of skeletons and a finite set of induced maps. Each induced map on a specific graph is represented by a non-negative integer matrix known as the incidence matrix. The objective, similar to Bestvina and Handel, is to find a graph and an induced map whose incidence matrix has the minimum Perron-Frobenius eigenvalue among all possible graphs and induced maps. 


Furthermore, when considering a homeomorphism $f$, J. Los identified three properties of an $f$-invariant train track that are crucial for $f$ to be isotopic to pseudo-Anosov (refer to \cite[Theorem 3.4]{los1993pseudo}). He then follows a finite number of steps, where he either finds an invariant train track for $f$ that satisfies the necessary conditions for the pseudo-Anosov class or determines that the class is not pseudo-Anosov.


The algorithm takes as input a braid $\beta \in B_n$, which is assumed to be given in \emph{minimal length form}. The author highlights the existence of an algorithm that, given a braid, can find a representative with minimal length using the Garside algorithm. However, it is noted that this method is not efficient due to its exponential complexity in relation to the initial length.
 
 
 By using a train track, it is possible to construct a Markov partition for $f$. Therefore, one consequence of Jerome's result is the existence of a coding for every pseudo-Anosov homeomorphism. However, as we will see, this coding is not sufficient to distinguish a conjugacy class from others. Nonetheless, it is a valuable corollary arising from his constructions.
 
 
  \subsection{Other Algorithms}
  
 There are certainly other classifications in the literature, but most of them focus on the classification modulo isotopy and its refinements.  However for the pseudo-Anosov case this is equivalent since two pseudo-Anosov homeomorphisms are isotopic if and only if they are topologically conjugated by a homeomorphism which is isotopic to the identity, the difference lies in the kind of arguments used for the classification. In the case of isotopy classification the authors use properties of foliations and homeomorphisms that are invariant under continuous deformations while we use arguments that highlight properties that are invariant under conjugation. 
 
 For instance, in the 1996 article by Hamidi et al. \cite{hamidi1996surface}, they present an algorithm that starts with a homeomorphism $f$ expressed as a combination of Dehn twists. The algorithm then determines whether $f$ is reducible or not. If it is reducible, it describes the isotopy classes fixed by $f$. If $f$ is pseudo-Anosov, the algorithm provides the contraction factor and invariant train tracks. Finally, if $f$ is periodic, it gives its period. These results offer additional insights and contribute to the overall understanding of surface homeomorphisms, up isotopy.
 

==> Realization/Algortmicgenimpasse.tex <==
\subsection{ Combinatorial formulation of finite genus and impasse}\label{Sub-sec: Comb Impasse genus}


The obstructions described above provide a valuable tool for analyzing our Markov partition from a visual perspective. However, in order to obtain an algorithmic characterization of the pseudo-Anosov class of geometric types, we need to translate these three topological obstructions and the impasse condition into a combinatorial formulation that allows us to determine in finite time whether or not these conditions are satisfied.

The key insight lies in Proposition \ref{Prop: properties ribbons}, where we observed that every ribbon of $k$-generation corresponds to the image of a horizontal strip between two consecutive horizontal sub-rectangles of the Markov partition for the map $\phi^k$ under the projection $\pi$. In this section, we will consider the geometric type.


$$
T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi_T:=(\rho_T,\epsilon_T )).
$$


The trick in our upcoming definitions is that whenever we want to talk about a "ribbon" with a certain property, we need to refer to two consecutive horizontal rectangles and analyze their images under $\phi^k$. This way, a "ribbon" is formed, and we can express the obstructions and the impasse property in terms of the images of these consecutive horizontal rectangles.

\subsubsection{Combinatorial obstructions for finite genus.}
\begin{defi}\label{Defi: Type 1 combinatoric}
	A geometric type $T$ satisfies the \emph{combinatorial condition} of type-$(1)$ if and only if there are:
	
	\begin{itemize}
		\item Three (not necessarily distinct) numbers, $k,i_0,i_1\in \{1,\cdots,n\}$.
		\item Three different  numbers, $l_0,l_1,l_2\in \{1,\cdots,v_{k}\}$ with $l_0<l_1<l_2$.
		\item A pair  $(k',l')\in\cV(T)$, such that $(k',l')\notin \{(k,l):l_0\leq l \leq l_2\}$.
		\item And four pairs, $(i_0,j_0),(i_0,j_0+1),(i_1,j_1)(i_1,j_1+1)\in \cH(T)$
		\end{itemize}
	Such that they satisfy one of the following relations:
\begin{enumerate}
\item If  $\rho_T(i_0,j_0)=(k,l_0)$ and $\rho_T(i_0,j_0+1)=(k,l_2)$, we have two available possibilities:
\begin{itemize}
	\item[i)] $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$.  In such a case:
	 $$
	 \rho_T(i_1,j_1)=(k,l_1), \, \epsilon_T(i_1,j_1)=1 \text{ and } \rho_T(i_1,j_1+1)=(k',l'),
	 $$
	  or well,
	  $$
	  \rho_T(i_1,j_1+1)=(k,l_1), \,  \epsilon_T(i_1,j_1+1)=-1,  \text{ and } \rho_T(i_1,j_1)=(k',l').
	  $$
	
	\item[ii)] $\epsilon_T(i_0,j_0)=-1$ and $\epsilon_T(i_0,j_0+1)=1$. In such a case  
	$$
	\rho_T(i_1,j_1)=(k,l_1), \,  \epsilon_T(i_1,j_1)=-1 \text{ and  }\rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
	\rho_T(i_1,j_1+1)=(k,l_1), \,  \epsilon_T(i_1,j_1)=1 \text{ and  } \rho_T(i_1,j_1)=(k',l').
	$$.
	
	
\end{itemize}
\item  In the symmetric case when, $\rho_T(i_0,j_0)=(k,l_2)$ and $\rho_T(i_0,j_0+1)=(k,l_0)$ there are two options:
\begin{itemize}
	\item[i)] $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$. In such a case: 
	$$
	\rho_T(i_1,j_1)=(k,l_1), \, \epsilon_T(i_1,j_1)=1  \text{ and }  \rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
	\rho_T(i_1,j_1+1)=(k,l_1), \, \epsilon_T(i_1,j_1+1)=-1  \text{ and }  \rho_T(i_1,j_1)=(k',l')
	$$

	\item[ii)]  $\epsilon_T(i_0,j_0)=-1$ and $\epsilon_T(i_0,j_0+1)=1$. In such a case:  
	$$
	\rho_T(i_1,j_1)=(k,l_1),\, \epsilon_T(i_1,j_1)=-1 \text{ and  } \rho_T(i_1,j_1+1)=(k',l')
	$$
	or well
	$$
\rho_T(i_1,j_1+1)=(k,l_1),\, \epsilon_T(i_1,j_1)=1 \text{ and  } 	\rho_T(i_1,j_1)=(k',l').
	$$
\end{itemize}
\end{enumerate}
	A geometric type has the \emph{combinatorial obstruction} of type-$(1)$ if there exists $m \in \mathbb{N}_{>0}$ such that $T^m$ satisfies the combinatorial condition of type-$(1)$.
\end{defi}


The way we have defined the combinatorial condition of type $(1)$ is by identifying the $1$-generation ribbons of the Markov partition $\cR_0$ in $\cR_1$ that give rise to the topological obstruction of type-$(1)$ in $\cR_1$ as the image of a horizontal stripe contained between two consecutive sub-rectangles. This understanding of ribbons corresponds to two consecutive elements $(i,j)$ and $(i,j+1)$ in $\cH$ and their images under $\rho_T$ in $\cV$, which represent the ribbons. In the following lemma we are going to follow the Figure \ref{Fig: Type one proof} to explain or proof. 


\begin{figure}[h]
	\centering
	\includegraphics[width=0.83\textwidth]{Preliminares/Imagenes/type1proof.png}
	\caption{Type $(1)$ combinatorial condition}
	\label{Fig: Type one proof}
\end{figure}



\begin{lemm}\label{Lemm: Equiv com and top type 1}
A geometric type $T$ has the combinatorial condition of type-$(1)$ if and only if the Markov partition in $\cR_1$ exhibits the topological obstruction of type-$(1)$.
\end{lemm}


\begin{proof}
The terms $(k,l_0)$, $(k,l_1)$, and $(k,l_2)$ represent three different vertical sub-rectangles of $R_k$ ordered by the horizontal orientation of $R_k$. The term $(k',l')$ represents a horizontal sub-rectangle of $\cR$ that is not located between the rectangles $V^k_{l_0}$ and $V^k_{l_2}$. Let's illustrate the meaning of the condition in the first case, as the rest are symmetric.

The conditions $\rho(i_0,j_0)=(k,l_0)$ and $\rho(i_0,j_0+1)=(k,l_2)$ are equivalent to the fact that the image under $f$ of the horizontal strip $\underline{H}_{j_0}$ bounded by $H^{i_0}_{j_0}$ and $H^{i_0}_{j_0+1}$ is a ribbon $r=f(\underline{H}_{j_0})$ of the first generation that connects the horizontal boundaries of $V^k_{l_0}$ and $V^{k}_{l_2}$. In this case, in Item $(i)$, the conditions $\epsilon_T(i_0,j_0)=1$ and $\epsilon_T(i_0,j_0+1)=-1$ means that the ribbon $r$ connects the upper boundary of $V^k_{l_0}$ with the upper boundary of $V^{k}_{l_2}$.

The conditions $\rho(i_1,j_1)=(k,l_1)$ and $\rho(i_1,j_1+1)=(k',l')$ indicate that the image of the strip $\underline{H}_{j_1}$ bounded by $H^{i_1}_{j_1}$ and  $H^{i_1}_{j_1+1}$ is a ribbon $r'$ connecting a horizontal boundary of $V^k_{l_1}$ with a horizontal boundary of $V^{k'}_{l'}$. Moreover, since $\epsilon_T(i_1,j_1)=1$, it means that $r'$ connects the upper boundary of $V^k_{l_1}$ with the stable boundary $\alpha$ of $V^{k'}{l'}$. But the condition $(k',l')\notin \{(k,l): l_0\leq l\leq l_2\}$ ensures that the stable boundary $\alpha$ cannot be situated between the upper boundaries of $V^k{l_0}$ and $V^k_{l_2}$, as we have specified from the beginning. Therefore the Markov partition $\cR_1$ have the topological obstruction of type $(1)$.

Is not difficult to see that if $\cR_1$ have the topological obstruction of type $(1)$, then the ribbons $r$ and $r'$ given by the definition \ref{Defi: Type 1 obstruction top}, are determined by be the image of a stripe comprised between consecutive sub-rectangles $H^{i_0}_{j_0}$ and $H^{i_0}_{j_0}$ for $r$ and $H^{i_1}_{j_1}$ and $H^{i_1}_{j_1+1}$ for $r'$. The rest of the conditions are totally determined.
\end{proof}





This coding method of representing a ribbon as two consecutive indices $(i,j)$ and $(i,j+1)$ in $\cH$ will be utilized frequently throughout this subsection. 


\begin{defi}\label{Defi: Type 2 combinatoric}
	The geometric type $T$ has the type-$(2)$ \emph{combinatorial condition} if and only if there are:
	\begin{itemize}
\item Four different pairs $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)\in \cV(T)$ with $l_1<l_2$ and $l^1<l^2$.
\item For pair $(i_1,j_1),(i_1,j_1+1),(i_2,j_2),(i_2,j_2+1)\in \cH(T)$ 
	\end{itemize}
Such that:
	$$
	\rho_T(i_1,j_1)=(k_1,l^1) \text{ and } \rho_T(i_1,j^1+1)=(k_2,l_2).
	$$
	
Additionally, depending on the signs of $\epsilon_T(i_1,j_1)$ and $\epsilon_T(i_1,j_1+1)$ we have the next constrictions:
	
	\begin{enumerate}
\item If $\epsilon_T(i_1,j_1)=\epsilon_T(i_1,j_1+1)$, then we have two options:
\begin{itemize}
\item[i)] If $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ then: $$\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)$$.

\item[ii)] If  $\rho_T(i_2,j_2)= (k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$. Then
$$-\epsilon_T(i_1,j_1)=-\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)$$.
\end{itemize}

\item If $\epsilon_T(i_1,j_1)=-\epsilon_T(i_1,j_1+1)$, then we have two options:

\begin{itemize}
\item[i)] If $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ then:
$$
\epsilon_T(i_2,j_2)=\epsilon_T(i_1,j_1) \text{ and  } \epsilon_T(i_2,j_2+1)=\epsilon_T(i_1,j_1+1).
$$
\item[ii)] If $\rho_T(i_2,j_2)=(k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$ then:
$$
\epsilon_T(i_2,j_2)=-\epsilon_T(i_1,j_1+1) \text{ and  } \epsilon_T(i_2,j_2+1)=-\epsilon_T(i_1,j_1).
$$

\end{itemize}

\end{enumerate}

\begin{comment}

$l'_1\in \{1,\cdots,l_1-1,l_1+1, v_{k+1}\}$ and $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ such that,  $l'_1<l_1$ if and only if  $l'_2>l_2$ and there are two options
$$
\Phi(i_2,j_2)=(k_1,l'_1,\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l'_2,\epsilon(i_2,j_2+2)) 
$$
or well
$$
\Phi(i_2,j_2)=(k_2,l'_2\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_1,l'_1,\epsilon(i_2,j_2+2)).
$$

\item Suppose $\epsilon(i_1,j_1)=-\epsilon(i_2,j_2+1)$. Then there are $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ and $l'_1\{1,\cdots,l_1-1,l_1+1v_{k+1}\}$ such that, $l'_1<l_1$ if and only if $l'_2<l_2$ and in this situation two possibilities are admissible:
$$
\Phi(i_2,j_2)=(k_1,l'_1,\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l'_2,\epsilon(i_2,j_2+2)) 
$$
or well
$$
\Phi(i_2,j_2)=(k_2,l'_2\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_1,l'_1,\epsilon(i_2,j_2+2)).
$$
\end{itemize}
\end{comment}


A geometric type $T$ has the \emph{combinatorial obstruction} of type-$(2)$ if there exists $m\in \NN$ such that $T^m$ satisfies the combinatorial condition of type-$(2)$.
\end{defi}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.83\textwidth]{Preliminares/Imagenes/tipp2pof.png}
	\caption{Type $(2)$ combinatorial condition}
	\label{Fig: Type two proof}
\end{figure}


 The Figure \ref{Fig: Type two proof} give some help to understand the proof.
 
\begin{lemm}\label{Lemm: Equiv com and top type 2} 
A geometric type $T$ satisfies the combinatorial condition of type-$(2)$ if and only if the Markov partition $\cR_0$ has the topological obstruction of type-$(2)$ on $\cR_1$.
\end{lemm}


\begin{proof}
The pairs $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)$ represent the respective vertical sub-rectangles of $\cR$ and the condition $\rho_T(i_1,j_1)=(k_1,l^1) \text{ and } \rho_T(i_1,j^1+1)=(k_2,l_2)$ implies the existence of a rubber $r=f(\underline{H}^{i_1}_{j_1})$ joining a pair of vertical boundaries of the rectangles $V^{k_2}_{l_2}$ and $V^{k_1}_{l^1}$ that correspond to the image  of the upper boundary of $H^{i_1}_{j_1}$ inside $V^{k_1}_{l^1}$ and the image of the inferior boundary of $H^{i_1}_{j_1+1}$ inside $V^{k_2}_{l^2}$.

In the situation when $\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)$ we can assume bot of them are positive (or negative, but the reasoning is the same). 

The condition: $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ implies that the rubber $r'=f(\underline{H}^{i_2}_{j_2})$ joints the stable boundary of $V^{k_2}_{l_2}$ that is the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ with the stable boundary $V^{k_1}_{l^1}$ that is the image  by $f$ of the upper boundary of $H^{i_2}_{j_2}$. 

Like $\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)$ this implies that $r$ joins the upper boundary of $V^{k_1}_{l^1}$ with the inferior boundary of $V^{k_2}_{l_2}$, even more like $$\epsilon_T(i_1,j_1)=\epsilon_T(i_2,j_1+1)=\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)=1$$
the $r'$ joins the upper boundary of $V^{k_1}_{l^2}$ (that is the image of the upper boundary of $H^{i_2}_{j_2}$) with the inferior boundary of $V^{k_2}_{l_1}$.
Like $l_1<l_2$ and $l^1<l^2$ the fist combinatorial condition implies that $\cR$ have a topological obstruction of type $(2)$.

Now if  $\rho_T(i_2,j_2)= (k_2,l_1)$ and $\rho_T(i_2,j_2+1)=(k_1,l^2)$, and 
$$\epsilon_T(i_2,j_2)=\epsilon_T(i_2,j_2+1)=-1$$,
The rubber rubber $r'$ have stable boundary in the upper boundary of $V^{k_1}_{l_2}$ as this correspond to the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ with the  inferior boundary of $V^{k_2}_{l_1}$ that correspond to the image by $f$ of the upper boundary of $H^{i_2}_{j_2}$. Therefore we have a type $(2)$ obstruction.

Consider now that $\epsilon_T(i_1,j_1)=-\epsilon_T(i_1,j_1+1)$. Too fix ideas  $\epsilon_T(i_1,j_1)=1$ and $\epsilon_T(i_1,j_1+1)=-1$. This means that $r$ joins the upper boundary of $V^{k_1}_{l^1}$ (that is the image by $f$ of the upper boundary of $H^{i_0}_{j_0}$)
with the upper boundary of $V^{k_2}_{l_2}$ (that correspond to the image by $f$ of the inferior boundary of $H^{i_1}_{j_2+1}$ ).

 The condition  $\rho_T(i_2,j_2)=(k_1,l^2)$ and $\rho_T(i_2,j_2+1)=(k_2,l_1)$ of the point $(2)$ in the definition together with:
 $$
\epsilon_T(i_2,j_2)=1 \text{ and  } \epsilon_T(i_2,j_2+1)=-1.
$$
implies that $r'$ joints the superior boundary of $V^{k_1}_{l^2}$ that is the image by $f$ of the upper boundary of $H^{i_1}_{j_1}$, with the upper boundary of $V^{k_2}_{l_2}$ that is the image by $f$ of the inferior boundary of $H^{i_1}_{j_1+1}$. Similarly we have the obstruction of type $(2)$ in the Markov partition.

Finally if  $\epsilon_T(i_1,j_1)=1$ and $\epsilon_T(i_1,j_1+1)=-1$ but now $\rho_T(i_2,j_2)=(k_2,l_1), \rho_T(i_2,j_2+1)=(k_1,l^2)$ and 
$$\epsilon_T(i_2,j_2)=1 \text{ and  } \epsilon_T(i_2,j_2+1)=-1.$$

we can deduce that $r'$ joints the upper boundary of $V^{k_1}_{l^2}$ that is the image by $f$ of the inferior boundary of $H^{i_2}_{j_2+1}$ and the upper boundary of $V^{k_2}_{l_1}$ that is the image by $f$ of the upper boundary of $H^{i_2}_{j_2}$. Once again we get a type two obstruction.

If the Markov partition $\cR$ have the type $(2)$ the ribbons $r$ and $r'$ determine the horizontal sub-rectangles determined by $(k_1,l^1),(k_1,l^2),(k_2,l_1),(k_2,l_2)$  and we can fix the condition 	$\rho_T(i_1,j_1)=(k_1,l^1)$ and $\rho_T(i_1,j^1+1)=(k_2,l_2)$ to indicate that $r$ joints such rectangles. The condition $(1)$ reflex the case when the two rectangles $R_{k_1}$ and $R_{k_2}$ have cohered orientation and the other case when they have inverse orientation. In any case, we need to remember that $r$ joint the image of the upper boundary of $H^{i_0}_{j_0}$ with the image of the inferior boundary of $H^{i_0}_{j_0}$. The four conditions enunciated are all the possible case when the ribbon $r'$ have stable boundaries in the same stables boundaries components of $\cR$ than $r$.

\end{proof}




\begin{defi}\label{Defi: Type 3 combinatoric}
A geometric type $T$ satisfies the \emph{combinatorial condition} of type-$(3)$ if there exist indices and conditions described as follows:
\begin{itemize}
\item Three numbers $k_1,k_2,k_3\in \{1,\cdots,n\}$ such that, for $\sigma=1,2$ or $3$:
\begin{eqnarray}
\Phi(k_{\sigma},1)=(k_{\sigma},l_{\sigma},\epsilon(k_{\sigma},1)=1) \text{ or }\\
\Phi(k_{\sigma},h_{k_{\sigma}})=(k_{\sigma},l_{\sigma},\epsilon(k_{\sigma},h_{\sigma})=1).
\end{eqnarray}
where $l_1\in \{1,\cdots,v_{k_{\sigma}}\}$.
\item A couple of numbers $1 \leq l_1'<l_1''<v_{k_1}$ such that: either $l_1'<l_1''<l_1$ or $l_1<l_1'<l_1''<l_1''$.
\item For $\sigma=2,3$, a number $l_{\sigma}'$ with $1\leq l_{\sigma}'\leq v_{k_{\sigma}}$, and
\item A pair of elements in $\cH$, $(i_2,j_2)$ and $(i_3,j_3)$.
\end{itemize} 
All of them complying with the following:
\begin{eqnarray}
\Phi(i_2,j_2)=(k_1,l_1',\epsilon(i_2,j_2)) \text{ and } \Phi(i_2,j_2+1)=(k_2,l_2',\epsilon(i_2,j_2+1)), \text{ or well }\\
\Phi(i_2,j_2+1)=(k_1,l_1',\epsilon(i_2,j_2+1)) \text{ and } \Phi(i_2,j_2)=(k_2,l_2',\epsilon(i_2,j_2)).
\end{eqnarray}
and at the same time:
\begin{eqnarray}
\Phi(i_3,j_3)=(k_1,l_1'',\epsilon(i_3,j_3)) \text{ and } \Phi(i_3,j_3+1)=(k_3,l_3',\epsilon(i_3,j_3+1)), \text{ or well }\\
\Phi(i_3,j_3+1)=(k_1,l_1'',\epsilon(i_3,j_3+1)) \text{ and } \Phi(i_3,j_3)=(k_3,l_3',\epsilon(i_3,j_3))
\end{eqnarray}
A geometric type $T$ has the \emph{combinatorial obstruction} of type-$(3)$ if there exists an $m\in \NN$ such that $T^m$ satisfies the combinatorial condition of type-$(3)$.
\end{defi}


\begin{lemm}\label{Lemm: Equiv com and top type 3}
A geometric type have $T$ has the combinatorial condition of type $(3)$ if and only if the Markov partition $\cR_0$ hs the topological obstruction  of type-$(3)$ on $\cR_1$. 
\end{lemm}


\subsubsection{The impasse property.}

Finally we proceed to formulate the impasse condition in terms of the geometric type.


\begin{defi}\label{Defi: Impasse combinatoric}
 Let $T$ be an abstract geometric type of finite genus. If $T=(m,\{(h_i,v_i)\}_{i=1}^n, \phi:(\rho,\epsilon):\cH\rightarrow \cV\times\{-1,1\})$, then $T$ has the \emph{impasse property} if there exist $(i,j),(i,j+1)\in \cH$ such that one of the following conditions holds:
 
\begin{eqnarray}
(\rho,\epsilon)(i,j)=(k,l,\epsilon(i,j)) \text{ and } (\rho,\epsilon)(i,j+1)=(k,l+1,-\epsilon(i,j)), \text{ or }\\
(\rho,\epsilon)(i,j)=(k,l+1,\epsilon(i,j)) \text{ and } (\rho,\epsilon)(i,j+1)=(k,l,-\epsilon(i,j)).
\end{eqnarray}
A geometric type $T$ has a \emph{combinatorial impasse} if there exists $m \in \mathbb{N}$ such that $T^m$ has the impasse property.
\end{defi}


Unlike the first three obstructions, where a ribbon is determined by two horizontal sub-rectangles and their respective indices $(i,j),(i,j+1)\in \mathcal{H}$, a topological impasse is defined in terms of a disjoint disk of $K$ and two arcs. Proving the equivalence between the topological and combinatorial formulations just given is a more subtle task, and we address it in the final part of this subsection.

\begin{theo}\label{Theo: Geometric and combinatoric are equivalent}
Let $T=(n,\{(h_i,v_i)\}_{i=1}^n,\Phi)$  be a geometric type of finite genus. Let $f: S \rightarrow S$ be a surface Smale diffeomorphism, and let $K$ be a saddle-type basic piece of $f$ that has a Markov partition of geometric type $T$. The following conditions are equivalent:

\begin{itemize}
\item[i)] The basic piece $K$ has a topological impasse.
\item[ii)] The geometric type $T^{2n+1}$ has the impasse property.
\item[iii)] The geometric type $T$ has a combinatorial impasse.
\end{itemize}
\end{theo}


\begin{proof}
 \textbf{ i) implies ii):} Let  $\cR=\{R_i\}_{i=1}n$ be a Markov partition of $K$ of geometric type $T$, and let $\overset{o}{D}$ be a topological impasse with $\alpha$ as the $s$-arc and $\beta$ as the $u$-arc, whose union forms the boundary of $D$.

 \begin{lemm}\label{Lemm: impasse disjoin int Markov partition}
The impasse is disjoint from the interior of the Markov partition, i.e.
$$
\overset{o}{D}\cap \cup_{i=1}^n \overset{o}{R_i}=\emptyset.
$$
Moreover, the intersection $\{k_1,k_2\}=\alpha\cap \beta$ is not contained in the interior of the Markov partition.
 \end{lemm}
 
\begin{proof}
Suppose that $\overset{o}{D}\cap \overset{o}{R_i}\neq \emptyset$. Let $\{k_1,k_2\}:=\alpha\cap \beta$ be the extreme points of the $s,u$-arcs on the boundary of $D$. There exists an unstable segment $J$ of $R_i$ such that $k_1\in J$. Moreover, $k_2$ is either in the interior of $J$ or on the stable boundary of $R_i$.  The second case is not possible since $k_2$ would be isolated from $K$ both from above and below, and there are no double $s$-boundary points in $K$. 


By similar arguments, we can conclude that $k_1$ and $k_2$ are in $\overset{o}{R_i}$. However, this leads to a contradiction as there would be a horizontal segment $I$ and a vertical segment $J$ of $R_i$ intersecting at two points in the interior of $R_i$ (namely $k_1$ and $k_2$). This is not possible, thus contradicting our assumption. Hence, $\overset{o}{D}$ is disjoint from the interior of $R_i$.

\end{proof}



If $\overset{o}{D}$ is an impasse, then $f^z(\overset{o}{D})$ is also an impasse for all integers $z \in \ZZ$. In the following lemma, we will construct a "well-suited" impasse that will make it easier for us to prove the first implication.

\begin{lemm}\label{Lemm: well suit impasse}
If $K$ has an impasse, then there exists another impasse $D'$ of $K$ such that the $s$-arc $\alpha'$ and the $u$-arc $\beta'$ on the boundary of $D'$ satisfy the following conditions:

\begin{itemize}
\item[i)]  $\beta'$ is in the interior of the unstable boundary of the Markov partition,  $\beta' \subset \overset{o}{\partial^u  \cR}$,
\item[ii)] $f(\beta')$ is not a subset of the unstable boundary of the Markov partition,  $\partial^u\overset{o}{\cR}= \overset{o}{\partial^u  \cR}$.
\item[iii)] $f^{2n+1}(\alpha)\subset \overset{o}{\partial^s \cR}$, where $n$ is the number of rectangles in the Markov partition.
\end{itemize}
\end{lemm}
 
 \begin{proof}
Let $D$ be an impasse of $K$ with $\alpha$ and $\beta$ as its boundary arcs. Let $\{k_1,k_2\}:=\alpha \cap \beta \subset K$ be the extreme points of these arcs. If $k_1$ is a periodic point, then there exists a positive iteration of $k_2$ that intersects $\alpha$ in its interior. However, this is not possible since the interior of $\alpha$ is disjoint from $K$. Therefore, we deduce that $k_1$ and $k_2$ are on the same stable separatrice of a periodic $s$-boundary point, and they are not periodic points themselves. Similarly, $k_1$ and $k_2$ are on the same unstable separatrice of a $u$-boundary point, but they are not periodic.

Since the negative orbit of $k_1$ converges to a periodic point $p_1$ on the stable boundary of the Markov partition, the negative orbit of $k_1$ approaches $p_1$ through points contained in the boundary of the Markov partition. Therefore, there exists $m \in \NN$ such that $f^{-m}(k_1)\in \overset{o}{\partial^u \cR}$.  We claim that if $f^{-m}(k_1)\in \overset{o}{\partial^u_{\epsilon}R_i}$, then $f^{-m}(k_2)$ is in the interior of the same unstable boundary component as $f^{-m}(k_1)$, i.e., $f^{-m}(k_2)\in \overset{o}{\partial^u_{\epsilon}R_i}$.

Indeed, since $f^{-m}(k_1)$ and $f^{-m}(k_2)$ are the boundary points of the $u$-arc $f^{-m}(\beta)$, there are no points of $K$ between them. The point $f^{-m}(k_1)$ lies in the interior of $\partial^u_{\epsilon} R_i$, which means that $f^{-m}(\beta)$ intersects the interior of this stable boundary component. This implies that $f^{-m}(k_2)$ is either an extreme point of $\partial^u_{\epsilon} R_i$ or lies in its interior, i.e., $f^{-m}(k_2) \in \overset{o}{\partial^u_{\epsilon}R_i}$.

If $f^{-m}(k_2)$ were an extreme point of $\partial^u_{\epsilon} R_i$, such an extreme point would not be surrounded by elements of $K$ on either side. This is because on one side we have the $u$-arc $f^{-m}(\beta)$, and on the other side it is on the unstable boundary of a rectangle in the Markov partition. However, this is not possible since $K$ has no double $s$-boundary points. Therefore, we conclude that $f^{-m}(k_2) \in \overset{o}{\partial^u_{\epsilon}R_i}$, as we claimed.


Now let us consider the impasse $D' = f^{-m}(D)$ instead of $D$. We will still use $\alpha$ and $\beta$ to denote the $s$-arc and $u$-arc on the boundary of $D$, but we assume that $\beta \subset \overset{o}{\partial^u \cR}$. Due to the uniform expansion along the unstable leaves, we know that there exists $m \in \NN$ such that $f^m(\beta) \subset \overset{o}{R_i}$, but $f^{m+1}(\beta)$  is no longer contain in  the unstable boundary of the Markov partition. Let us define $D' = f^{m}(D)$ with boundary arcs $\alpha'$ and $\beta'$. This impasse satisfies items $i)$ and $ii)$ of our lemma, since $\beta'$ is contained in the interior of $\overset{o}{\partial^u \cR}$ and $f(\beta')$ is not a subset of $\partial^u \overset{o}{\cR} = \overset{o}{\partial^u \cR}$.


In view of Lemma \ref{Lemm: impasse disjoin int Markov partition}, the points $f(k_1)$ and $f(k_2)$ are not in the interior of the Markov partition. We conclude that $f(k_1)$ and $f(k_2)$ belong to $\partial^s \cR$ because both are on the boundary of $\cR$ but not inside the unstable boundary. By the invariance of the stable boundary of $\cR$ under positive iterations of $f$ and the Pigeonhole principle applied to the $2n$ components of stable boundaries of the Markov partition, we know that $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ lie on periodic stable boundaries of the Markov partition. Moreover, $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ lie on the same stable separatrice, and on each separatrice, there is a single stable boundary component of $\cR$ that is periodic (even though they are all pre-periodic). This implies that $f^{2n}(f(k_1))$ and $f^{2n}(f(k_2))$ are in $\overset{o}{\partial^s_{\epsilon}R_j}$ for a single stable boundary component of the rectangle $R_j$. This proves item $iii)$ of our lemma.

\end{proof}



With the simplification of  Lemma \ref{Lemm: well suit impasse} we deduce that $\beta\subset \partial^u R_i$ and $f^{2n+1}(\alpha)\subset \partial^s R_k$. 

Let us consider the partition $\cR$ viewed as a Markov partition of $f^{2n+1}$. We claim that $\beta$ is an arc joining two consecutive sub-rectangles of $(\cR,f^{2n+1})$, denoted as $H^i_j$ and $H^{i}_{j+1}$. In effect, $\beta$ is a $u$-arc joining two consecutive rectangles or is properly contained in a single sub-rectangle $H$ of $(\cR,f^{2n+1})$. This is because the stable boundaries of $H$ are not isolated from $K$ within $H$, as would be the case if the ends of $\beta$ were on the stable boundary of $H$. Therefore, the only possibility is that $\beta$ is properly contained in a rectangle $H$. In this case, $f^{2n+1}(H)$ is a vertical sub-rectangle of $R_i$ containing $f^{2n+1}(\beta)$ as a proper interval. However, the endpoints of $f^{2n+1}(\alpha)$, which coincide with the endpoints of $f^{2n+1}(\beta)$, are not in the interior of the stable boundary of $R_k$, which contradicts the hypothesis. Thus, we conclude that $\beta$ joins two consecutive sub-rectangles.


Let $H^i_{j}$ and $H^i_{j+1}$ be the consecutive rectangles joined by $\beta$. Suppose that $f^{2n+1}(H^i_j)=V^k_{l}$ with the change of vertical orientation encoded by $\epsilon_{T^{2n+1}}(i,j)$ and $f^{2n+1}(H^i_{j+1})=V^k_{l'}$ with the change in the vertical orientation encoded by $\epsilon_{T^{2n+1}}(i,j+1)$. Between $V^k_{l}$ and $V^k_{l'}$ there are no points of $K$ because the $s$-arc $f^{2n+1}(\alpha)$ joins them in the horizontal direction, this implies that $l'\in \{l+1,l-1\}$. The vertical orientation of $\beta$ is the same as $H^i_j$ and $H^i_{j+1}$, furthermore $f^{2n+1}(\beta)$ joins the horizontal sides of the rectangles $V^k_{l}$ and $V^k_{l'}$ which are on the same stable boundary component of $R_k$,  this implies that the vertical orientation of $f(H^i_j)$ is the inverse of the orientation on $f(H^i_{j+1})$ within $R_k$ (to visualize this it suffices to follow the segment $f^{2n+1}(\beta)$ with a fixed orientation), thus $\epsilon_{T^{2n+1}}(i,j)=-\epsilon_{2n+1}(i,j')$.


The geometric type of the Markov partition $\cR$ for the map $f^{2n+1}$ is $T^{2n+1}$. Our construction implies that $T^{2n+1}$ has the impasse property. With this, we conclude the first implication of the theorem..


 \textbf{ ii) implies iii):} The geometric type $T^{2n+1}$ has the impasse property, which implies that $T$ has a combinatorial impasse.
 

\textbf{ iii) implies i):} Suppose $T^m$ has the impasse property. Let $H^i_j$ and $H^i_{j+1}$ be consecutive horizontal sub-rectangles in the Markov partition $\cR$ for the map $f^{m}$, as given by the impasse property. This condition implies that if $f^{2n+1}(H^i_j)=V^k_{l}$ and $f^{2n+1}(H^i_{j+1})=V^k_{l'}$, then $l$ and $l'$ are consecutive and have inverse vertical orientations.


The stable segments of on the stable boundary of $R_k$ between $V^k_{l}$ and $V^k_{l'}$ do not contain elements of the maximal invariant set of $f^m\vert_{\cR }$, since they are consecutive sub-rectangles of the partition $\cR$ seen as a Markov partition of $f^m$. In fact they do not contain elements of $K$ since $K=f^m(K)$ and therefore those segments are $s$-arcs of $f$. Furthermore, the image by $f^{m}$ of the two arcs $u$ on the boundary  of $R_i$ that join $H^i_j$ and $H^i_{j+1}$ are $u$-arcs of $f$. Between the two pairs of arcs there is an $s$-arc $\alpha$ and a $u$-arc $\beta$ such that they intersect each other only at their ends. We affirm that $\alpha$ and $\beta$ delimit a disk $D$ with a disjoint interior of $K$.


Suppose that $\gamma:=\alpha \cup \beta$ does not bound a disk. This means that $\gamma$ is not homotopically trivial, and neither are its iterations $\{f^m(\gamma)\}{m=1}^{\infty}$. In fact, since the stable segments of such curves lie in the stable manifold of a periodic point, there exists a $k\in \NN$ such that $\{f^{mk\}(\gamma)}{m=1}^{\infty}$ is a set of disjoint curves. We will argue that two of these curves are not homotopic, leading to a contradiction with the fact that the surface $S$ where the basic piece is contained has finite genus.

\begin{lemm}\label{Lemma: gamma not homotopic imagen}
The curve $\gamma$ is not homotopic to any other curve $f^{2mk}(\gamma)$ for $k\in \mathbb{N}$.
\end{lemm}


\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{Preliminares/Imagenes/Anillo.png}
	\caption{ The Annulus}
	\label{Fig: The annulus}
\end{figure}


\begin{proof}
Suppose $\gamma$ and $f^{m}(\gamma)$ are homotopic, which means they bound a topological annulus $\AA$ in $S$. Let us endow the boundary of $\AA$ with the clockwise orientation, and assume that $\gamma$ represents the interior boundary of $\AA$, while $f^m(\gamma)$ represents the exterior boundary.

Then, under the map $f^m$, a small sub-annulus $\mathcal{A}'$ of $\mathcal{A}$, which has $\gamma$ as one of its boundary components, is mapped to another annulus $f^m(\mathcal{A}')$, where $f^m(\gamma)$ serves as a boundary component. Here is the key point: if $f^m(\gamma)$ preserves the clockwise orientation, we can make $\mathcal{A}'$ small enough so that the interior of $f^m(\mathcal{A}')$ is disjoint from $\mathcal{A}$.


Suppose $f^m$ reverses the clockwise orientation of $\gamma$. We emphasize that $\gamma$ and $f^{2m}(\gamma)$ are still homotopic and bound an annulus $\mathcal{A}$. However, in this case, $f^{2m}$ preserves the clockwise orientation of the inner boundary. Hence, there exists a small sub-annulus $\mathcal{A}'$ of $\mathcal{A}$ that is bounded by $\gamma$, and the interior of $f^{2m}(\mathcal{A}')$ is disjoint from $\mathcal{A}$. Therefore, we can assume that $\gamma$ and $f^{2km}(\gamma)$ satisfy this property.

Suppose that $\gamma$ is saturated by the hyperbolic set $K$ in the interior direction of $\AA$, and therefore, it is isolated from $K$ in the exterior direction of $\AA$. Then $f^{2km}(\gamma)$ is isolated from $K$ in the interior direction of $\AA$ and saturated by $K$ in the exterior direction of $\AA$. In particular, there exists $x\in K \cap (S \setminus \AA)$.
 
Since ${k_1, k_2}$ and ${f^m(k_1), f^m(k_2)}$ are not periodic points, they do not have free separatrices. Moreover, $k_1$ and $k_2$ lie on the same separatrice. Without loss of generality, let's assume that $k_1$ has a stable separatrice $I$ that does not connect it to a periodic point. The separatrice $I$ cannot remain entirely inside $\AA$ because there exists a point $x \in K$ outside of $\AA$. Non-free separatrices of points $y \in K$ that do not connect $y$ to a periodic point are dense in $K$, so $I$ needs to approach $x$ arbitrarily closely. The boundary of $\AA$ is the union of four arcs, which means that the separatrice $I$ cannot intersect them in their interiors. Therefore, the possible scenarios are as follows:

 \begin{itemize}
\item The intersection point is $k_2$, which is impossible since it would imply that $I$ is inside a closed leaf of $W^s(K)$,
\item The other point is $f^m(k_1)$ or $f^m(k_2)$. This is not possible because in that case, $I$ would need to be contained in the separatrice of $f^m(k_1)$ (or $f^m(k_2)$), which is not the same as the $s$-arc in $f^{2km}(\gamma)$. But this separatrice points towards the exterior of $\AA$
 \end{itemize}
 
So, $I$ couldn't intersect either $f^m(\gamma)$ or $\gamma$. We conclude that $I$ is a subset of $\AA$, which is a contradiction. This ends our proof.
 
\end{proof}

Then, if $\gamma$ is not null-homotopic, we could find an infinite amount of disjoint and non-isotopic curves (See \cite[Lemma 3.2]{juvan1996systems}), which is a contradiction with the finite genus of the surface $S$. It follows that $\gamma$ bounds a disk.


\begin{coro}\label{key}
	
	The disk bounded by $\gamma$ doesn't intersect $K$.
\end{coro}

\begin{proof}
If there exists $x \in K \cap \overset{o}{D}$, then $x$ has at least one non-free stable separatrice $I$. Such a separatrice is not confined within $D$ because there exist points in $K$ that are not in $D$ (they are those on the other side of the $s$-arc $\alpha$ on the boundary of $D)$. Additionally, $I$ is dense in $K$. Therefore, $I$ must intersect the $u$-arc $\beta$ on the boundary of $D$. However, the separatrice $I$ does not intersect the extreme points $\{k_1,k_2\}=\alpha \cap \beta$ because no local separatrices of them intersect the interior of $D$. This leads to a contradiction. Hence, $K \cap \overset{o}{D} = \emptyset$.
\end{proof}



This implies that $D$ is an impasse for $f$.



\end{proof}

\subsection{Algorithmic Determination of Finite Genus and Impasse }\label{Sub-sec: algoritm finite genus}


The objective is to prove the following proposition that will serve as the key element in determining, algorithmically and in finite time, whether a geometric type belongs to the pseudo-Anosov class or not. In the future, we will derive the property of double boundaries from the fact that the incidence matrix of a geometric type in the pseudo-Anosov class is mixing. Therefore, we formulate this property as the first one to be verified.

\begin{prop}\label{Prop: mixing+genus+impase is algorithm}
	Given any abstract geometric type $T=(n\{(h_i,v_i),\},\Phi)$, there exists a finite algorithm that can determine whether $T$ satisfies the following properties:
	\begin{enumerate}
		\item The incidence matrix of $T$, $A(T)$ is mixing. 
		\item The genus of $T$ is finite.
		\item  $T$ exhibits an impasse.
	\end{enumerate}
	Furthermore, the number of iterations of $T$ required by the algorithm to determine these properties is upper bounded by $6n$, where $n$ represents the size of $T$.
\end{prop}



\begin{proof}
	
	We have formulated specific conditions on the combinatorics of $T$ to determine whether $T^n$ has an impasse or one of the three obstructions to have finite genus. Furthermore, according to Theorem \ref{Theo: finite type iff non-obstruction}, determining whether or not $T$ has finite genus requires computing at most $T^{6n}$. To determine whether $T$ has an impasse, Theorem \ref{Theo: Geometric and combinatoric are equivalent} states that it is necessary to compute at most $T^{2n+1}$. Since $n\geq1$, it is clear that $2n+1<6n$, which provides the upper bound we claim in the proposition. Proposition \ref{Prop: algorithm iterations type} asserts that the computation of $T^{6n}$ is algorithmic, thus confirming the existence of an algorithm to determine the finite genus and the presence of an impasse for $T$.
	
	
	
	
	We have left the mixing criterion for last. The following lemma is the basis for the upper bound on the number of iterations to verify the mixing of the incidence matrix.
	
	\begin{prop}\label{Prop: bound positive incidence matriz }
		If $A$ is a non-negative mixing matrix of size $n \times n$, then $A^n$ is positive definite.
	\end{prop}
	
	\begin{proof}
		
		Consider the directed graph $\mathcal{G}$ with $n$ vertices corresponding to the matrix $A$. In this graph, there is an edge pointing from vertex $v_i$ to vertex $v_j$ if and only if $a_{ij} > 0$ in the matrix $A$. Since $A$ is mixing, it means that there is always a path from any vertex $v_i$ to any other vertex $v_j$ in the graph $\mathcal{G}$.
		
		To prove our Lemma, it is sufficient to demonstrate that there exists a path of length less than or equal to $n$ between any two vertices in the graph.
		
		
		
		Consider a path $\gamma = [v_{i(1)}, \cdots, v_{i(m)}]$ from $v_i = v_{i(1)}$ to $v_j = v_{i(m)}$ in the graph $\mathcal{G}$. Let $\gamma$ have $m$ vertices and be of minimum length among all paths connecting these vertices.
		
		If any two vertices of the path $\gamma$ are equal, it implies the existence of a cycle within $\gamma$. We can eliminate this cycle and obtain a new path $\gamma'$ from $v_i$ to $v_j$ with a shorter length than $\gamma$. This contradicts the assumption that $\gamma$ has the minimum length. Hence, all vertices in $\gamma$ must be distinct.
		
		Therefore, the length of $\gamma$ is necessarily less than or equal to $n$, since there are only $n$ distinct vertices in the graph.
	\end{proof}
	
	
	If $T$ is in the pseudo-Anosov class, we have $A^n(T) = A(T^n)$. According to the previous Lemma, if $A(T)$ is a non-negative matrix, then $A(T^n)$ is positive definite. This implies that $A(T^n)$ is mixing and does not have double boundaries. Therefore, for a given geometric type $T$ with $A(T)$ being a non-negative matrix, the positivity of $A(T^n)$ is equivalent to its mixing property, which in turn implies the absence of double boundaries.
	
	\begin{coro}\label{Coro: algoritmic mixing}
		Given a geometric type $T$, if $A(T^n)$ is not positive definite, then $T$ is not in the pseudo-Anosov class.
	\end{coro}
	
	Clearly, we only need to iterate $T$ $n$ times, and the upper bound given in the proposition remains valid. 
	This concludes our proof.
\end{proof}

==> TotalInvariant/SubEulerandType.tex <==
\section{The Euler characteristic and the geometric type}\label{Sec: euler characteristic}

 For now lets point some result of independent importance. Previously we didn't demand a  knowledge of the surface $S$ where of pseudo-Anosov homeomorphism $f$ acts, instead, by assuming that $S$ accepts a pseudo-Anosov homeomorphism of geometric type $T$ we  could deduce the Euler characteristic of of $S$. The core of our analysis is the \emph{Euler-Poincare formula}:
 
 \begin{prop}\label{Prop; Euler Poincare formula}[Euler-Poincare formula]
 	Let $S$ be a closed surface with a singular foliation $\cF$. Let $P_s$ be the number of prongs at a singular point $s$. Then
 	$$
 	2\chi(S)=\sum_{s\in \text{Sing}(\cF)}(2-P_s).
 	$$
 \end{prop}
 

  Let $f:S\rightarrow S$ be a pseudo-Anosov homeomorphism with measured foliations $(\cF^s,\mu^s)$ and $(\cF^u,\mu^u)$ in this section we assume that:
\begin{itemize}
\item $S$ is a closed surface with finite set of marked points $P\subset S$.
\item $f:S\rightarrow S$ is a pseudo-Anosov homeomorphism with all their spines contained in $P$.
\item The set of singularities of $f$ is denoted as Sing$(f)$.
\end{itemize}

\subsection{The pictorial algorithm}

Let $T$ be a geometric type in the pseudo Anosov class, we are going to see in  Chapter \ref{Chapter: Realization}  that $T$ admits  a realization by disjoint rectangles, $(\cR'=\{R_i\}_{i=1}^{n},\Phi')$. This result is independent of this section, so we are going to assume the existence of such family.
Let $0\leq m\leq 4n'$ a natural number such that every periodic boundary point of $\Phi'$  and every separatrice in the boundary of the rectangles in $\cR'$ are fixed by $\phi$. 


Let $f:S\rightarrow S$ be a pseudo-Anosov homeomorphism with a Markov partition of geometric type $T$, then  $T^m$ is the geometric type of a Markov partition of $f^m:S \rightarrow S $  and then  is in the pseudo-Anosov class, therefore $T^m$  and admits a realization by disjoint rectangles $(\cR=\{R_i\}_{i=1}^n,\phi)$. We should use this realization to calculate the genus of $S$.


Let $p\in R_i$ a fixed stable boundary point and be $I\subset\partial^s R_i$ be a stable separatrice of $p$, we could deduce what other separatrice $I'$ is identify with $I$ in the next manner.

Let ${V^i_l}_{l=1}^L$ the set of vertical sub-rectangles of $R_i$ which have an stable boundary intersecting whose interior intersect $I$. Suppose that for all $l$ :
$$
V^i_l=\Phi(H^{i(l)}_{j(l)}).
$$ 

The stable separatrice $I$ is necessarily identify with another separatrice $I'$, then there is at lest one $l\in \{1,\cdots, L\}$ such that: there exist $j'\in \{1,\cdots, v_{i(l)}\}\setminus\{j(l)\}$ such that if:
$$
\Phi^(H^{i(l)})_j'=V^{i'}_{l'}
$$
 and,  if the interior of (upper) inferior boundary $I_-$ of $H^{i(l)}_{j(l)}$ is such that $\Phi(\overset{0}{I_-})\cap  \overset{o}{I}\neq \emptyset $ then the interior of the (inferior) upper boundary $I_+$  of $H^{i(l)})_j'$ satisfy that $\phi(\overset{o}{I_+})\cap I'\neq \emptyset$. This procedure determines unequivocally the separatrices that are identified. This construction allows us to know how many stable separatrices the point $p$ has, i.e. we have been able to calculate $P_p$. This graphical description permits to calculate the Euler characteristic using a draw of the rectangles, this is why we call it pictorial algorithm.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{TypeConjugacy/Imagenes/sepindetify.pdf}
	\caption{Two stable segments.}
	\label{Fig: Two segments}
\end{figure}

\subsection{The symbolic algorithm.}

Let $T$ a geometric type in the pseudo-Anosov class, let $(\Sigma_T,\sigma_T)$ it combinatorial model, be  $\cR={R_i}_{i=1}^n$ a a Markov partition of $\Sigma_T$ of geometric type $T$. Let $\pi:\Sigma_A \rightarrow \Sigma_T$ the semi-conjugation. We recall some definitions and result of our previous section:
\begin{itemize}
 \item The set of $s,u$-periodic boundary points of $(\Sigma_A,\sigma)$ is calculated using the $s,u$-boundary generating function ( see ~ \ref{Defi: s-boundary generating funtion}). Even more, like we are looking for boundary periodic points, it period is at most $2n$, then it is enough to applied such function $2n$ times, for ever pair $i_0\in \{1,\cdots,n\}$ and $\epsilon_0=\pm 1$, which is finite set. We fix the notation:
 $$
 Per_{s,u}(A)=\{\underline{w}\in \Sigma_A: \underline{w} \text{ is a } s,u-\text{periodic boundary code } \}
 $$
 and 
 $$
  Per_{B}(A)= Per_{s}(A)\cup  Per_{u}(A).
 $$
 \item The set of $s,u$-periodic boundary points of $\Sigma_T$ is obtained by:
 $$
 Per_{s,u}(T)=Per_{s,u}(A)/\sim_T.
 $$
It calculation is algorithmic as $\sim_T$ is determined algorithmically.
 \item The function, $\pi:\sigma_A \rightarrow \Sigma_T$  is determine by $\sim_T$ and then it definition is algorithmic.
\end{itemize}


Let $[w]\in Per_B(T)$, suppose that $[w]$ have $k$-prongs, the set of admissible codes that project to $[w]$ is $\pi^{-1}([w])=\{\underline{w_j}\}_{j=1}^m$, every one of this codes is an \emph{sector code} of $[w]$, then $m\leq 2k$. If fact if $[w]$ is in the corner of every rectangle $R_i\subset \Sigma_T$ that contains $[w]$, $m=2k$. Then
$$
P_{[w]}=\frac{m}{2}.
$$
But suppose that $[w]$  is a $s$-boundary periodic point of $\sigma_T$ that is in the interior of the stable boundary of a rectangle $R_i$, then, there is two sector codes of $[w]$ that are equal, like the number of prong of $[w]$ is equal to $\frac{1}{2}$ of the amount of sector codes  of $k$ we could define the following function:
$$
a(\underline{w}) =
\begin{cases}
1 & \text{if } w\in Per_{s}(A)\cap Per_u(A)  \\
2 & \text{if } w\in Per_{s}(A)\setminus Per_u(A) \cup  Per_{u}(A)\setminus Per_s(A)  
\end{cases}
$$

and then we calculate $P_[w]$ as:
$$
\frac{1}{2}P_[w]= \sum_{\underline{w}\in \pi^{-1}([w])}a(\underline{w}).
$$


Once we have the previous information we could use Euler-Poincare formula to determine the Euler characteristic and we obtain the following result.



\begin{coro}\label{Coro: Algorithm to Euler characteritic}
Let $T$ be a geometric type in the pseudo-Anosov class, and let $f:S\rightarrow S$ be a generalized pseudo-Anosov homeomorphism with a geometric Markov partition of type $T$. There exists a finite algorithm that, given $T$, determines the number of $k$-prongs of $f$ (for every $k\geq 0$) and the Euler characteristic of $S$.
\end{coro}




